C-AllOut: Catching & Calling Outliers by Type

Given an unlabeled dataset, wherein we have access only to pairwise similarities (or distances), how can we effectively (1) detect outliers, and (2) annotate/tag the outliers by type? Outlier detection has a large literature, yet we find a key gap in the field: to our knowledge, no existing work addresses the outlier annotation problem. Outliers are broadly classified into 3 types, representing distinct patterns that could be valuable to analysts: (a) global outliers are severe yet isolate cases that do not repeat, e.g., a data collection error; (b) local outliers diverge from their peers within a context, e.g., a particularly short basketball player; and (c) collective outliers are isolated micro-clusters that may indicate coalition or repetitions, e.g., frauds that exploit the same loophole. This paper presents C-AllOut: a novel and effective outlier detector that annotates outliers by type. It is parameter-free and scalable, besides working only with pairwise similarities (or distances) when it is needed. We show that C-AllOut achieves on par or significantly better performance than state-of-the-art detectors when spotting outliers regardless of their type. It is also highly effective in annotating outliers of particular types, a task that none of the baselines can perform.

==> paper_CatchOutAll copy/1_introduction.tex <==
\section{Introduction} \label{sec:intro}

%%%%%\reminder{What is the problem?}

This work considers a novel outlier mining problem: Given an unlabeled point-cloud dataset (wherein we may have access {only} to the pairwise similarities, or distances, between points---as opposed to feature representations), we propose \method to (1) effectively detect (``catch'') the outliers, and also (2) tag/annotate (``call'') the outliers by their \textit{type}.








Outlier mining is a useful task for many applications, for which a vast body of detection techniques exists
%and has therefore  a large literature %, with various detection techniques broadly classified as those based on distances, density, statistical modeling, clustering, angles, subspaces, etc.
\cite{han2012outlier}.
Despite this popularity, we identify a key gap in the literature: methods that not only can detect, but also \textit{annotate the type of the outliers detected}. % they detect}.  
%Outliers are often categorized as three types:
Point-cloud datasets exhibit three main types of outliers: global, local (or contextual), and collective (or clustered), as illustrated in {Fig. \ref{fig:crown_input_output}(a).}
While several existing methods \cite{inne,lof,kriegel2008angle,outrank,loci} may potentially detect all three types of outliers, they do not label or annotate them \textit{explicitly}. The typical output of the existing detectors in the literature is either a binary label (outlier/inlier), or an overall outlierness score per point---not an ``outlier label'', i.e. an annotation reflecting its type. In fact, (to our knowledge) there is no existing detection algorithm that can annotate outliers of all types. We found SRA \cite{nian2016auto} to be the closest attempt, % to ranking outliers by type,
however, it provides a \textit{single} ranking along with a binary flag: scattered vs. clustered. This does not adequately address the task (See related work in \S\ref{sec:related}), and performs poorly in experiments (\S\ref{sec:experiments}). 

\begin{figure}[!t]
\begin{tabular}{cc}
        \includegraphics[width=0.375\linewidth]{images/data.pdf}
       &
        \includegraphics[width=0.575\linewidth]{images/rankings.pdf} \\
        (a) example input & (b) example output
        \end{tabular}
        \vspace{-0.1in}
    \caption{\small{(a) Example toy data with inliers (circles) and 3 types of outliers (stars): global (red), local (green), and collective (black);  (b)
    Existing methods provide an overall outlier ranking, regardless of type.
    \method also provides separate rankings for outlierness by type.
    }}
    \label{fig:crown_input_output}
    \vspace{-0.25in}
\end{figure}

%%\reminder{Is it an important problem? Why? Who cares?}
As outliers are key indicators of faults, inefficiencies, malicious activities, etc. in various systems, outlier annotations could provide valuable information to analysts for sensemaking, triage and troubleshooting. Global outliers can be interpreted as the most severe yet isolate cases that do not repeat; e.g., a human mistake that occurred while typing the value of an attribute, say to register value $10$ instead of $1.0$.
Local ones are outliers with respect to a specific context, like a particularly short basketball player that could be seen as an inlier among non-players, or a hot day in the winter that may be interpreted as usual within days from other seasons.
Finally, collective outliers may be critical for settings such as fraud detection, indicating coalition or repetitions, as compared to isolate `one-off' outliers. For example, they could be attacks that exploit the same loophole in cyber systems, or bots under the same command-control.%to illegitimately defame or promote a product in e-commerce.
%\reminder{we may want to beef up why and to-whom annotations matter.}

%annotations: global vs local gives information about the severity, local implies contextual, collective may be more valuable for some settings such as fraud detection as compared to `one-off' outliers.


%%\reminder{Is it a trivial problem? What makes it hard?}

Annotating outliers by \textit{type} -- as global, local, or collective -- is a more general, and a strictly harder problem than mere detection.
Even though it is a categorization task, it remains an \textit{unsupervised} one, provided that the detection task/dataset itself does not contain any labels. 
While one may think of segmenting the detected outliers by a given detector into various types {\em post-hoc} (i.e., proceeding detection), how to do so is not obvious.
%To take advantage of classification would not be an option here, as there are no labels available.
Intuitively, a post-hoc annotation procedure would require knowledge about the clusters of similar points within the entire dataset; this would both define the potential contexts for local outliers and allow the identification of microclusters formed by points with high outlierness scores, so to treat them as collective outliers.
However, clustering itself is a hard task; most of the existing algorithms require user-defined parameters, like the number of clusters $k$ in $k$-means or the minimum density ${MinPts}$ in DBSCAN \cite{ester1996density}, and still struggle with cases where the clusters have arbitrary shapes and/or distinct densities, or even when the data has no clusters at all.
These are probably the main reasons why we do not see any attempts of post-hoc annotation of outliers in the literature.
%\reminder{x-pacs: explanations in groups..}



%Only similarities are given - 

%%%%%\reminder{What has been done so far? Why is it not sufficient?}

We remark that
(to the best of our knowledge) the problem of annotating outliers has not been addressed by any prior work. Notably our solution is \textit{self-contained}, that is, we do not treat this problem as a separate, post-hoc attempt, but rather propose a new outlier detection approach, called \method, that can {\em simultaneously detect  and annotate} all three types of outliers in point-cloud datasets.
%\reminder{we may try some post-processing to do this task as baselines. can mention such post-hoc approaches are not as effective.}
%On the other hand, solely similarity-based detection has been studied and in fact, 
%In terms of similarity-based detection, 
%various existing methods based on $k$-nearest-neighbor distances \cite{lof,knn} directly apply. 
%%%%There exist similarity based methods - some are space and time inefficient, requiring the all-pairs similarities.
%To our knowledge, there is no existing method that (at least explicitly) annotates the detected outliers by type.
%\reminder{What is new here? List of Contributions.}
%Contributions are two-pronged : a novel detection model that can work only with similarities and can also provide outlier annotations 
Specifically, \method\ builds on the Slim-tree~\cite{slimtree}, an efficient data indexing structure with log-linear time complexity, that queries only $O(n\log n)$ pairwise similarities between points for construction. Based on this data structure, we introduce novel measures that are capable of effectively quantifying the outlierness of each point by type; as global, local or collective outlier.


%%\reminder{Is it an important problem? Why? Who cares?}
As a by-product, our work can handle outlier mining settings for which \textit{only pairwise similarities can be accessed}, i.e., data points do not reside in an explicit feature space, but the similarity between any pair of points can be queried.
This setting may arise in domains with complex objects, such as galaxies, cellular tissues, etc., where providing (relative) similarities between objects may be more intuitive or convenient for domain experts than explicitly denoting them with specific feature values.
Privacy-sensitive domains, such as medicine and finance, are other settings where pairwise comparison (of patients, customers, etc.) may be deemed less risky than revealing their explicit feature values.
While our work concerns this setting, we are not limited by it; for traditional settings
%in which features are explicitly given for the objects can also be handled easily, 
where points lie in an explicit feature space, pairwise similarities can easily be computed  
provided a meaningful similarity function. 

%Of course, \method\  where data in a feature space can easily be used to compute pairwise similarities directly.


%%\reminder{Is it a trivial problem? What makes it hard?}

%similarity-based detection: it may be hard to depict complex objects, e.g. galaxies, with explicit features but may be more intuitive or convenient for domain experts to provide (relative) similarities between objects.



 
We summarize our main contributions  as follows.



\cbit 

\item{\bf New outlier mining algorithm:} We introduce \method, a novel ``catch-n-call'' algorithm that can not only effectively detect but also annotate the outliers by type. To our knowledge, no existing work addresses the outlier annotation problem.


\item{\bf Annotating outliers:}  %first method to annotate all three types of outliers 
Given a point-cloud, \method 
creates four separate rankings
%of the points 
(See {Fig. \ref{fig:crown_input_output}(b)}): an overall ranking, as well as rankings that reflect global, local and collective outlierness; all of which are estimated efficiently from the same underlying data structure  \method builds on.
%In other words, \method can rank the points in four respective ways. 
%It raises a flag when it does not find any outliers of a specific type or  any outliers at all.

\item{\bf Other desirable properties:} 
Besides providing outlier annotations, \method exhibits several other desirable properties for practical use. First, it is parameter-free and requires no user input.
Moreover it is scalable, with log-linear time complexity %\reminder{space complexity??} 
for model construction and outlier scoring.
Finally, it can handle scenarios where only
pairwise similarities between points are available (but not explicit feature representations), while not being restricted to this setting.

\item{\bf Effectiveness \& New  benchmark datasets:} We evaluate \method against  state-of-the-art detectors 
%, including LOF \cite{lof}, one-class SVM \cite{scholkopf2000support}, $k$NN \cite{knn}, and %ensemble based iForest \cite{liu2008isolation}, 
where it achieves on par or significantly better performance on standard benchmark datasets.  On additional carefully designed testbeds with annotated outliers, we also show the efficacy of \method at outlier annotation---a task none of the baselines can address. On comparable results (only), \method is superior to SRA \cite{nian2016auto}. 
%\gs{iForest here should be changed to SIF \cite{czekalski2021similarity}}
\ceit 

To foster future work on the outlier annotation problem and for reproducibility, we open source \method, all benchmark datasets with annotated outliers and data generators, at \url{https://bit.ly/3iUVwtM}.

%{\bf Reproducibility:}

%\todo{we should have a table of symbols; it helps to standardize the notation}

%The rest of the paper follows a traditional organization:
%related work~(\S\ref{sec:related}),
%preliminaries and background~(\S\ref{sec:back}),
%proposed method~(\S\ref{sec:method}),
%experiments~(\S\ref{sec:experiments}),
%and conclusions~(\S\ref{sec:conclusion}).
%\input{paper_CatchOutAll/symbols}







==> paper_CatchOutAll copy/2_related.tex <==
\section{Related Work} \label{sec:related}

%\la{add SRA; as most closely related. also shrink text.}
Outlier mining has a  large literature on detection algorithms as it finds applications in numerous real world domains \cite{books/sp/Aggarwal2013}. % such as environmental monitoring, cybersecurity, finance, healthcare and medicine, to name a few.
%Therefore, there is a  . 
Our work concerns algorithms for point-cloud data, where existing detectors can be categorized in various ways; e.g. based on  %the
employed measures %that they employ, 
such as 
distance-, density-, angle-, depth- etc.,  %Another is 
or by the modeling approach %that they use, 
such as 
statistical-modeling, clustering,
ensemble, subspace, etc. among many others \cite{han2012outlier}.
%There are also detectors 
%They can also be organized by the nature of input data \cite{chandola2009anomaly},  such as   streaming \cite{gupta2013outlier},  %\cite{conf/ijcai/TanTL11,conf/kdd/ManzoorLA18}, 
% high-dimensional \cite{zimek2012survey}, and distributed \cite{angiulli2012distributed} %,yan2017distributed,tsou2018robust}
% outlier detection.

Here we discuss detection algorithms under a different light, i.e. with respect to \textit{outlier types}, % (instead of the measures or models that they use or the nature of data they can handle),  
as our work  focuses on detecting \textit{and annotating} outliers by type.
Namely, point-cloud datasets may contain three types of outliers: global (or gross), local (or contextual/conditional), and collective (or clustered/group).

Most detection algorithms assume outliers to be scattered, isolated points that are far from the majority \cite{knorr1998algorithms,kriegel2008angle,knn,scholkopf2000support}.
Such outliers are referred to as global outliers or gross anomalies.
A second class of detectors target contextual outliers, defined as points that are different under a certain context \cite{liang2016robust,conf/pkdd/MeghanathPA18}. These %are also referred to as conditional outliers \cite{song2007conditional,conf/aaai/HongH16}, and 
can be seen as %a type of 
local outliers that deviate locally \cite{lof,dang2013local,kriegel2009loop}. A third category of methods focus on  collective outliers, defined as
groups of points that collectively deviate significantly from the rest, even if the
individual members may not be outliers \cite{han2012outlier}.

Note that specialized techniques  for outliers of certain types often also detect other types, without differentiating them by type. For instance, LOF  \cite{lof} for local outlier detection also gives large, if not larger, scores to global outliers. % in a dataset.
Similarly,  $k$NN  \cite{knn} would give large outlier scores to collective outlier points provided $k$ is larger than the size of the collective group. In fact, all of these methods are evaluated on classical benchmark datasets w.r.t. \textit{overall} detection performance. 
On the other hand, there are techniques specifically designed to detect all three types of outliers \cite{inne,lof,kriegel2008angle,outrank,loci}. 
However none of these approaches provides any means for annotation.
{Our proposed \method is designed exactly to fill this gap in the literature.}

The closest work to ours is the SRA algorithm \cite{nian2016auto} with key distinctions. Unlike \method, it provides only a \textit{single} ranking, along with a binary flag to indicate if the ranking reflects clustered or scattered outlierness (not both).  Moreover, for the latter, it does not distinguish between global and local outliers. 





\hide{
While specialized techniques have been designed to detect outliers of certain types, as discussed above, it is not to conclude that they will {\em only} detect those types. % of outliers.
For instance, LOF algorithm \cite{lof} for local outlier detection also gives large, if not larger, scores to global outliers in a dataset.
Similarly,  $k$NN algorithm \cite{knn} would give large outlier scores to collective outlier points provided $k$ is larger than the size of the collective group.
Thus existing methods, while being able to detect certain types of outliers, often also detect other types in the process, without differentiating them by type (recall that no existing method provides outlier annotations). In fact, all of these methods are evaluated on classical benchmark datasets w.r.t. \textit{overall} detection performance. 
Even if these specialized methods detected only the types of outliers they were originally designed for, there would be no single all-around (i.e. ``one-stop shop'') method to detect all and any type of outliers \textit{with} annotations.
{Our proposed \method is designed exactly to fill this gap in the literature.}
}

Besides annotating outliers, \method exhibits 
%Next we discuss related work in terms of 
other desirable properties, %of \method, 
namely it is parameter-free, scalable, and uses solely pairwise similarities.
In comparison, most
%Most 
outlier detectors exhibit user-defined (hyper)parameters (HPs), % to be set by the users,
e.g. number of nearest neighbors (NNs) $k$ for NN-based methods \cite{lof,knn}, distance threshold \cite{knorr1998algorithms}, %threshold for 
fraction of outliers \cite{knorr1998algorithms,scholkopf2000support}, 
etc. %, number of ensemble components for ensemble models \cite{iforest,loda}, etc.
It is understood that most detectors are quite sensitive to their HP choices % of their HPs
\cite{goldstein2016comparative}, however, it is unclear how to set them since hold-out/validation data with ground-truth labels simply does not exist for unsupervised detection. 
Moreover, the most prevalent techniques are distance- or density-based and rely on NN distances which are either expensive to compute or need to be approximated \cite{lof,knorr1998algorithms,loci,knn,scholkopf2000support}.  
Finally, as we motivated in the previous section, various detection algorithms that work % with points 
in an explicit feature space are not suitable for settings where only the pairwise similarities can be provided e.g. for privacy or expert convenience reasons. 
Unfavorably, 
it is the $k$-NN based methods that can readily handle pairwise similarities, which however are computationally demanding and sensitive to the choice of their HP(s).
We remark that \method is free of these practical challenges, while addressing the novel outlier annotation problem for the first time.



%parameters - e.g. DB-Outlier \cite{knorr1998algorithms}


%scalable



%pairwise



==> paper_CatchOutAll copy/3_background.tex <==
\section{Problem Statement \& Preliminaries} \label{sec:back}


Considering (to the best of our knowledge) \method is the first solution to outlier annotation, we first  formalize the problem. We also %give background on
describe Slim-trees; the  underlying data structure that \method builds on.

\subsection{Problem Statement~}
\vspace{-0.05in}
%The outlier annotation problem is formally defined as the following.

\begin{Definition}
[\textbf{Outlier Annotation Problem}]{Given a point-cloud  dataset $\dataset=\{ \point{1}, \dots, \point{n} \}$ in which only the distances, or similarities, $\distij$ between any two objects $\pointi$ and $\pointj$ can be accessed; 
Provide four types of ranking of the objects by outlierness:
1) $\orank$, an \textit{overall} ranking of outliers regardless of their type; as well as 
a ranking by 2) \textit{global}, 3) \textit{local}, and 4) \textit{collective} outlierness, respectively denoted by 
$\grank$, 
$\lrank$, and
$\crank$.
\label{definition:problem}
}
\vspace{-0.05in}
\end{Definition}


\begin{Definition}[\textbf{Ranking of Outliers}]{
A ranking of outliers $\rank=( r_1, r_2, \dots, r_n )$ is a permutation of the set $\{1, 2, \dots, n\}$. It defines an ordering of the instances in a dataset $\dataset=\{ \point{1}, \dots, \point{n} \}$ by separating the outliers
$\{\point{r_1}, \point{r_2}, \dots, \point{r_m}\}$ from the inliers $\{\point{r_{m+1}},\point{r_{m+2}}, \dots,$ $\point{r_n}\}$, where $m \ll n$ is the number of outliers in $\dataset$.
\label{definition:ranking}
}\end{Definition}

%\la{i think this is a good place to roughly describe what global, local, collective mean. hard to give formal definition, but we can point to  fig. 1 to informally describe here in text. }



%\reminder{notation and definitions (?): global, local, collective}


\subsection{Slim-tree~} \label{sec:slimtree}
%\la{Start with overall structure. Layer-wise nodes, hierarchically organized, single root, multiple children. etc.}

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{\linewidth}
%        \includegraphics[width=0.9\linewidth]{images/data_leaves.pdf}
%        \caption{Data having leaf representatives (triangles) with their radius of action. Remaining points (circles and stars) are indexed by those representatives.}
%        \label{fig:crown_data_leaves}
%    \end{subfigure}
%    \begin{subfigure}{\linewidth}
%        \centering
%        \includegraphics[width=0.9\linewidth]{images/data_root.pdf}
%        \caption{Data having the single root object (square) with its radius of action. Other points (circles and stars) are indexed by this root object.}
%        \label{fig:crown_data_root}
%    \end{subfigure}
%    \caption{Three-leveled Slim-tree structure obtained using the data presented in Figure \ref{fig:crown_input_output}.}
%    \label{fig:crown_data_tree}
%\end{figure}

Slim-tree~\cite{slimtree} is a tree-based data structure.
It relies solely on distances (or similarities) $\distij$ between pairs of objects $\pointi, \pointj \in \dataset$, and can be built in $O(n \log n)$ time using any metric distance function for point-cloud data in a feature space.
The distances can be either given to the tree without using features, or computed directly from them.
%As it happens with other structures of its category, which are known as Metric Access Methods, Slim-tree 
%It uses solely distance calculations between objects that are embedded in a metric space.
%A metric space is defined as a pair $\langle \mathbb{X}, d \rangle$, where $\mathbb{X}$ is the data domain and $d : \mathbb{X} \times \mathbb{X} \xrightarrow{} \mathbb {R}$ is the distance function used to compare objects from $\mathbb{X}$.
%The following properties must hold for any objects $x_i, x_j, x_k \in \mathbb{X}$:
%\begin{enumerate*}[label=(\alph*)]
%    \item non-negativity, $0 \leq d(x_i, x_j) < \infty$;
%    \item identity, $d(x_i, x_j) = 0 \iff x_i = x_j$;
%    \item symmetry, $d(x_i, x_j) = d(x_j, x_i)$, and;
%    \item triangle inequality, $d(x_i ,x_j) \leq d(x_i, x_k) + d(x_k, x_j)$.
%\end{enumerate*}
%The aforementioned setting applies to many data domains and distance functions, including multidimensional objects to be compared with an $L^p$-norm, like the Euclidean distance.

A tree~$\tree$ has nodes organized hierarchically into levels.
As shown in Def.ns~\ref{definition:root}, \ref{definition:leaf}, \ref{definition:anc} and~\ref{definition:rep},
tree $\tree$ has always one single root node $\rootnode$.
Root $\rootnode$ stores into a set $\rootpoints$ at most $c \in \mathbb{Z}^+$ objects from dataset $\dataset$, where $c$ is the maximum node capacity.
Each object $\repany \in \rootpoints$ is said to be the representative of a child $\node$ of the root; thus, root $\rootnode$ has $|\rootpoints|$ children.
Node $\node$ also follows the same structure: it stores into a set $\bN$ at most $c$ objects from $\dataset$.
It is always true that $\rootpoints \cap \bN = \{ \repany \}$, which means that $\repany$ is the one and only object stored redundantly both in $\node$ and in its direct ancestor $\antany=\rootnode$.
Note that $\repany$ is always nearby the \textit{most centralized object} in $\bN$.
%Additionally, it is correct to say that $\antany=\rootnode$ is the direct ancestor of node $\node$.
This organization continues recursively with node $\node$ having $|\bN|$ child nodes, each of which also having children of its own, until reaching a leaf node $\leafname$.
Leaf $\leafname$ has the same structure of any other node, except that it has no children.
Note that every object $\pointi \in \dataset$ is stored into the set $\leafipoints$ of one and only one leaf $\leafi$.
\vspace{-0.05in}
\begin{Definition}[Root] {
The root node $\rootnode$ of a tree $\tree$ built for a dataset $\dataset$
%=\{ \point{1}, \point{2}, \dots, \point{n} \}$ 
is the single node existing at the highest level of $\tree$.
The set of (root) objects stored in $\rootnode$ is denoted by $\rootpoints$%\la{O inherently suggest Outlier set, it may be confusing. Shall we use a different letter?}
, where $\rootpoints \subseteq \dataset$. %and $|\rootpoints| \leq c$.
\label{definition:root}
}
\vspace{-0.05in}
\end{Definition}

\begin{Definition}[Leaf] {
The leaf node of an object of interest $\pointi \in \dataset$ 
%within a dataset $\dataset=\{ \point{1}, \point{2}, \dots \point{n} \}$  \la{$\pointi \in \dataset$?} 
in a tree $\tree$ is the only node $\leafi$ existing at the lowest level of $\tree$ such that $\pointi \in \leafipoints$, where $\leafipoints \subseteq \dataset$ is the set of objects stored in $\leafi$.
%\la{denoted}
%Let us refer to this node as
%It is denoted by $\leafi$.
%\la{$\leafi$?}.
\label{definition:leaf}
}\end{Definition}


\begin{figure}[!th]
\begin{tabular}{cc}        \includegraphics[width=0.44\linewidth]{images/data_root.pdf}
       &
        \includegraphics[width=0.44\linewidth]{images/data_leaves_latex_font.png} \\
        (a) root node & (b) leaf nodes
        \end{tabular}
        \vspace{-0.1in}
    \caption{Tree $\tree$ for the toy data in Fig. \ref{fig:crown_input_output}(a) of \S\ref{sec:intro}. 
    %Each root object in (a) represents one leaf node in (b).
    }
    \label{fig:tree}
    \vspace{-0.2in}
\end{figure}


\vspace{-0.05in}
\begin{Definition}[Direct Ancestor] {
The direct ancestor node $\antany$ of a node $\node \neq \rootnode$
%\la{$\node \neq \rootnode$} 
within a tree $\tree$ %indexing a dataset
%\la{just $\dataset$, do you even need to mention X here?} $\dataset=\{ \point{1}, \point{2}, \dots \point{n} \}$ 
is the node that directly points to $\node$ from the previous level of $\tree$. 
Note that $\ant{\rootnode}$ is undefined for root node $\rootnode$.
%if $\node \neq \rootnode$ \la{remove, included above};  otherwise, it is undefined. \la{remove, simply say it is undefined or unspecified for the root $\rootnode$?}
\label{definition:anc}
}
\vspace{-0.05in}
\end{Definition}

\vspace{-0.05in}
\begin{Definition}[Representative] {
The representative object $\repany \in \dataset$ of a node $\node \neq \rootnode$ in a tree $\tree$ built for a dataset $\dataset$ %=\{ \point{1}, \point{2}, \dots \point{n} \}$ 
is the only object both in $\node$ and in $\antany$.
Note that $\rep{\rootnode}$ is undefined for root node $\rootnode$.
%For simplicity of notation, let $\repi$ be the representative of a leaf $\leafi$ \la{but this is i's leaf. not any leaf.}, i.e., $\repi = \rep{\leafi}$.
%\la{this definition is confusing to me. even after revision.}
%\rc{Leman, please, check if it is better now.}
\label{definition:rep}
}
\vspace{-0.05in}
\end{Definition}

Fig.~\ref{fig:tree} shows a tree $\tree$ built for the toy data in Fig. \ref{fig:crown_input_output}(a) of \S\ref{sec:intro}. 
Each of the $3$ root objects in (a) represents one leaf node in (b).
One of them is leaf $\leafi$ with radius $\lradiusi$. Object $\pointi$ is in $\leafi$;
its nearest neighbor is $\nni$.



%The tree is built in a bottom-up manner by following a procedure that resembles the construction of the well-known structure B$^+$-tree.
%The objects are initially inserted into a single root node until a predefined maximum node capacity $c$ is reached.
%Once a new object arrives for insertion, one of the most central objects among the objects in the root is elected to be a representative.
%Then, the root is split into two leaf nodes; and, the representative is promoted to be stored into a new node created to replace the previous root,
%so the tree grows one level.
%This process is repeated recursively by inserting new objects in leaf nodes and, whenever a node becomes full, splitting it into two new nodes and promoting a representative to a higher level in the tree.
%The result is a height-balanced tree structure that stores all objects in leaf nodes, while having in each internal node copies of the most representative objects among the ones in the corresponding subtree. 
%Figure~\reminder{\ref{fig:slimtree}} illustrates one Slim-tree created with \reminder{$c=X$} for the toy dataset that we used as a motivational example in the introductory section.

%\la{ 2-d figure with examples to the above definitions}

%A Slim-tree node is a cluster of objects. An index node is a node that stores only other index nodes or leaf nodes, no objects. A leaf node is a node that stores only objects, no nodes. A subtree is the slice of the tree that considers only the currently analyzed node and its child nodes. The first level of the tree, the root level, has only the root node and it cannot have parent nodes. The second to last level of the tree, the leaf level, is the last level before the object level and it cannot have child nodes, it can only store objects. The object level is a conceptual level where there are only objects and no nodes. Inner levels of the tree may have both index or leaf nodes.

%In this paper we refer to data instances, interchangeably, as points, objects, observations and instances.

%\reminder{earlier there was separation here}



%\todo{I believe that we could have in the introduction the synthetic dataset that Guilherme has been working on; then, the toy data could be item (a) of the figure, while the corresponding Slim-tree would be item (b).}



==> paper_CatchOutAll copy/4_proposed.tex <==
\section{Proposed Method} \label{sec:method}

%This section introduces \method;
% we first give a general overview highlighting its main steps, and then present the details for each of these steps.


\subsection{\method in a Nutshell~}
%This section provides a high-level overview of our proposed algorithm \method.
The main idea behind our method is to tackle the outlier annotation problem by leveraging the information present in a tree-based indexing structure, namely the Slim-tree.
Particularly, \method takes advantage of the ability of this data structure to group together similar instances and keep apart distinct instances, with varying ``degrees'' of similarity being captured by means of distinct tree levels.
The pseudocode of \method is in Algo.~\ref{algorithm:main}.

In line with the problem statement in Def.n~\ref{definition:problem}, \method receives a dataset $\dataset$ as input, and  produces four rankings of outliers $\orank$, $\grank$, $\lrank$ and $\crank$, respectively reflecting outlierness overall, as well as global, local and collective outlierness.
A parameter $\maxiter \in \mathbb{Z}^+$ is also received as input, for which we provide a reasonable default value $\maxiter=10$ to free \method from user-defined parameters.
The default value is based on a comprehensive empirical evaluation, see  \S\ref{ssec:refine}.

In a nutshell, \method has two main phases.
It begins in Phase~$1$ with a data-driven procedure that automatically creates and fine-tunes the base tree structure; see Lines~$1$-$9$ in Algo.~\ref{algorithm:main}. In this phase, we perform %in this phase one
an iterative refinement of the tree which is controlled both by the overall ranking produced from preliminary trees, as well as by the maximum number of iterations $\maxiter$.
Once a fine-tuned tree is obtained, Phase~$2$ takes place; see Lines~$10$-$12$ in Algo.~\ref{algorithm:main}. It extracts from the refined tree the information required to rank outliers by type, and produces the final output.
The next two subsections give details on each of these phases. % our method.

%\reminder{Algorithm with pointers to subsequent subsections}

\begin{algorithm}[!t]
{\small{
\caption{\method}
\label{algorithm:main}
\textbf{Input} Dataset $\dataset=\{ \point{1}, \point{2}, \dots \point{n} \}$;
%\\ \hspace*{10mm} 
maximum number of iterations (default: $\maxiter=10$)\\
\textbf{Output} Overall ranking $\orank$; 
%\hspace*{13mm} 
Global ranking $\grank$; 
%\hspace*{13mm} 
Local ranking $\lrank$; 
%\hspace*{13mm} 
Collective ranking $\crank$.
\begin{algorithmic}[1]
%\State 
\LineComment{\textcolor{blue}{Phase $1$: building and refining the tree}}
\State $\rank \gets (1, 2, \dots n)$;
\Comment{given order of objects}
\For{$i = 1, 2, \dots \maxiter$}
    \State $\tree \gets $ {\sc CreateTree($\dataset$, $\rank$)};
    \State $\orank \gets $ {\sc Overall($\dataset$, $\tree$)}; \Comment{ Ranking~\ref{definition:overall} (\S\ref{sec:overall})}
    \If{$\orank == \rank$}
        \State \textbf{break};
    \EndIf
    \State $\rank \gets \orank$;
\EndFor
\LineComment{\textcolor{blue}{Phase $2$: outlier-type focused ranking of objects}}
\State $\grank \gets $ {\sc Global($\dataset$, $\tree$)}; \Comment{ Ranking~\ref{definition:global} (\S\ref{sec:global})}

\State $\crank \gets $ {\sc Collective($\dataset$, $\tree$)}; \Comment{ Ranking~\ref{definition:collective} (\S\ref{sec:collective})}
\State $\lrank \gets $ {\sc  Local($\dataset$, $\tree$)}; \Comment{ Ranking~\ref{definition:local} (\S\ref{sec:local})}

\State \Return $\orank, \grank, \lrank, \crank$;
\end{algorithmic}
}}
\end{algorithm}
\setlength{\textfloatsep}{0.15in}

\vspace{-0.05in}
\subsection{Building and Refining the Tree}

%Distance-based outlier detection is a popular approach to detect outliers due to its ease of understanding and adaptivity. 
%Clusters can be formed using any distance calculations that can return a dissimilarity level between two given objects. 
%Indexing structures, like the Slim-tree, have the ability to group instances together using indexes. These groups can be seen as clusters, as two instances of data need to be similar to be indexed together. Based on this notion, we suggest that the Slim-tree can be used as a sort of hierarchical clustering algorithm. 

%The main idea behind our method is to tackle the outlier annotation problem by exploiting the information within a tree-based indexing structure, namely the Slim-tree.
%This section describes how we %propose to 
We build and refine a Slim tree as the base to both rank and annotate the outliers. % the tree that is used as a base to annotate outliers \la{let's stick to outlier and not anomaly for consistency.}.
%Traversing the tree we can choose any needed hierarchy level of the clustering. (the idea around this paragraph should be improved)
%On lower levels, (higher levels or lower levels? need to make the paper text use only one the same notation for this) of the tree, 
%on leaf nodes for example, the size of the subsample is very small and it holds only instances that are closely related to each other. 
For construction, the tree relies solely on pairwise distances (or similarities), and
can be built using any metric distance function for point-cloud data in a feature space.
This property also makes \method  applicable to settings where only distances between objects are available, but not explicit features.
Importantly, not all but only $O(n\log n)$ pairwise distances are required for construction, making it scalable to large datasets.

% As such, 

% there are two options to employ it in a dataset:
% \begin{enumerate*}[label=(\alph*)]
% \item to provide the pairwise distances between each object to be inserted in the tree and \la{what is the second part about? node representatives are also provided? confusing.} the node representatives along its path of insertion from the root down to one of the leaves; or
% \item to compute these distances directly from the data features.
% \end{enumerate*}
% In our work we choose option (a), since we are considering a setting where just distances are available, not features.
% Nonetheless, \method also works and gives the same results whenever features and the appropriate distance function are provided.

%Having the objects put into the tree, we can perform certain comparisons between the objects to determine outlierness scores for the documents. 
%Taking into consideration the previously defined outlier types, we have come up with one technique capable of identifying all types of outliers and three other techniques that can be used to independently detect global, local and collective outliers.

In the following two subsections, we (1) describe how 
%The next subsection shows how 
to use the tree to create an overall outlierness ranking of the objects, which
 is then used to (2) improve/re-construct the tree structure by ensuring that inliers are more likely to be inserted early on.
%\la{this sentence is almost repeat of 1st sentence of 4.2.1 below. drop one.}
%Later, we exploit it to improve one initial tree into a fine-tuned one.
%\la{a brief intuition as to what fine-tune means would be helpful: ``we use the overall ranking of instances to adjust the insertion order such that inliers are more likely to be inserted early on.''? this assumes background section will talk about insertion and how order can be important.}


\subsubsection{Overall Ranking of Outliers}\label{sec:overall}

%The Slim-tree is structured using the objects themselves in its leaf and index nodes. Each level of the tree has selected representative objects that are somewhat centralized in their nodes. This means that recursively, every representative object is located more or less at the center of not only its node, but also, in a central position of all other objects indexed in its subtree. In that sense, we can say that every representative object represents a subsample of the data. Leaf nodes represent the smallest subsample, having only objects closely related to each other. Parent nodes of leaves encompass all of the objects contained in the closer leaves. So, the parent node representative object represents a larger subsample of the data, having objects not so closely related to each other, but still having a fair share of similarities.
%Following this logic, we can say that the representative of the root node, although not always being the most central object, lies within the most centralized area of the entire set of objects present in the Slim-tree.

%This section shows how to take advantage of the base tree structure to rank outliers regardless of their types. 
Our overall ranking $\orank$ %is given i~\ref{definition:overall}, which 
%Note that it 
is based on two structural components of the tree in 
Def.ns~\ref{definition:croot} and~\ref{definition:frep} which are presented first.
%in this subsection, besides the tree-based Definitions~\ref{definition:root}, ~\ref{definition:leaf}, ~\ref{definition:anc} and~\ref{definition:rep} from the previous Subsection~\ref{sec:slimtree}.

%It comes from the ability of the tree to create data-driven samples of the dataset, with varying ``degrees'' of similarity being considered by means of distinct tree levels, and recognizinh  

\vspace{-0.05in}
\begin{Definition}[Closest Root Object]{
The closest root object $\crooti$ %\la{double x confusing, see below} 
of an object $\pointi \in \dataset$ %within a dataset $\dataset=\{ \point{1}, \point{2}, \dots, \point{n} \}$ 
inside a tree~$\tree$ is given by
%the object $\pointj \in \rootpoints$ that minimizes the distance $\distij$.
$\crooti := \{\pointj \in \rootpoints \;|\; \arg\min_j \distij\}$.
%\la{can't we write this formally as $\crooti := \{\pointj \in \rootpoints \;|\; \arg\min_j \distij\}$?}
\label{definition:croot}
}
\vspace{-0.05in}
\end{Definition}

\begin{Definition}[Foreign Representative]{\sloppy{The foreign representative $\frepi$ %\la{double x is confusing, can't we simplify to $\point^{(i)}_{\mathtt{f}}$? -- best to make $\backslash$newcommand} 
of an object  $\pointi \in \dataset$ %within a dataset $\dataset=\{ \point{1}, \point{2}, \dots \point{n} \}$ \la{$\pointi \in \dataset$ should be enough? no need to list 1 through n} 
indexed by a tree $\tree$ is given by $\frepi := \{\pointj \in \bE \ | \ \arg\min_j \distij\}$, where
%the object $\pointj \in \bN$ that minimizes the distance $\distij$, 
$\bE = \{ \repany \;|\; \node \in \tree \ \land \ \antany = \anti \}$.} \label{definition:frep}
%\la{the last notation is complicated; 3 nested subscripts is too much. simplify to $\alpha_{\leafi}$?} 
}\end{Definition}


%\la{It would be good if we could separate standard definitions like Root, etc. from paper-specific definitions like Overall Ranking. Any ideas?}

\begin{ranking}[\textbf{Overall Ranking}]{
The overall ranking of outliers $\orank = ( r_1, r_2, \dots, r_n )$ for a dataset $\dataset=\{ \point{1}, \dots, \point{n} \}$ indexed by a tree $\tree$ is 
the ranking in which $\oscore{r_i} \geq \oscore{r_{i+1}} \ \forall i \in \{ 1,2,\dots, n-1\}$, where
%the outlier scoring function $\oscorename : \dX \xrightarrow{} \mathbb{R}$ is given by
\vspace{-0.1in}
\begin{equation}
\label{eq:overall_score}
 \oscorej = \dist{\pointj}{\crootj} \ \cdot \ \dist{\pointj}{\frepj}
\end{equation}
\label{definition:overall}
\vspace{-0.3in}
}\end{ranking}
The main idea %behind our proposal
is to leverage the set of objects $\rootpoints$ that are stored in the root node~$\rootnode$ of the tree $\tree$ built from the input dataset $\dataset$, 
by 
%being the first ones (to our knowledge) to 
recognizing that $\rootpoints$ is in fact a small and data-driven sample (i.e., subset of objects from $\dataset$)  containing only the objects from $\dataset$ that best summarize the main clusters of inliers.
As described in \S\ref{sec:slimtree}, the leaf nodes of $\tree$ store all the objects in $\dataset$, with each leaf having only objects that are very similar to each other.
Distinctly, an internal node solely has one object from each one of its child nodes: the most centralized object in the child.
%The selection of the most centralized object is more detailed or more general according to the level of $\tree$. %\la{Robson to refine}
%The radius of each internal node is as large as it is needed to cover every object of its ; 
It means that any internal node is essentially a cluster of clusters.
Notably, the information in the tree closely resembles the output of a hierarchical clustering algorithm.

As a consequence, it is reasonable to expect that an object $\pointi \in \dataset$ that clearly belongs to a cluster of inliers tends to be the one selected as the representative $\repi$ of its leaf node $\leafi$, and then again selected to be the representative 
%$\rep{\anti}$ 
of the direct ancestor $\anti$ of leaf $\leafi$, and still continue being selected as a representative up to the root node $\rootnode$, thus becoming a member of set~$\rootpoints$.
This line of thought lead us to believe that each object in $\rootpoints$ represents one of the clusters of inliers  in $\dataset$, where the larger is the cluster, the more representatives it has\footnote{Note that $\rootpoints$ typically has a few hundreds of objects, so we expect $k \ll |\rootpoints|$, where $k$ is the number of inlier clusters in $\dataset$.}.
Following Def.n~\ref{definition:croot}, let $\crooti$ be the object in $\rootpoints$ that is the closest to an object of interest~$\pointi$. For short, we simply say that $\crooti$ is the closest root object of $\pointi$.
Note that it helps us to distinguish outliers from inliers: if $\pointi$ is an inlier, then it tends to be closer to $\crooti$ than it would be if it were an outlier.

Nonetheless, some small clusters of inliers may be underrepresented in the root node.
In this particular case, the distance to the closest root object becomes less helpful.
%In that case, if this inlier cluster is somewhat isolated, all of its inlier objects are going to be interpreted as outliers. 
Fortunately, there also exists the tendency that a cluster of inliers requires more than one leaf node to be stored, since any tiny cluster that fits entirely into a single leaf is more likely to contain collective outliers than inliers.
This tendency also helps us to distinguish outliers from inliers: if an object $\pointi$ is close to at least one leaf other than leaf $\leafi$, it tends to be an inlier; otherwise, $\pointi$ is probably an outlier.
Following Def.n~\ref{definition:frep}, we efficiently take advantage of this idea through the concept of foreign representative~$\frepi$ of an object $\pointi$.
The overall ranking of outliers $\orank$ shown in Ranking~\ref{definition:overall} builds on the aforementioned concepts by using a new score $\oscorei$ as a base.
It capitalizes on the proximity of an object $\pointi$ both to its closest root object~$\crooti$ and to its foreign representative~$\frepi$ to accurately and efficiently rank outliers of any type.
%\la{add 1-2 sentences re: why it is efficient. b/c there are logarithmically few root objects? what about \#representatives?}

%where:
%\begin{enumerate*}[label=(\alph*)]
%\item each cluster has exactly one representative, when $k = |\rootpoints|$;
%\item some clusters have more than one representative each, when $k < |\rootpoints|$, or;
%\item small clusters have no representative, when $k < |\rootpoints|$.
%\end{enumerate*}
%Therefore, the distance $\mathtt{d}(\pointi, \point_{\mathtt{o}(\pointi)})$ between any object of interest $\pointi$ and its closest root object $\point_{\mathtt{o}(\pointi)}$ is a fair indicator of the outlierness of $\pointi$.
%Inliers tend to have small distances; larger distances occur for local outliers, and there should exist even larger ones for global and collective outliers.




%that a cluster that is large enough to be considered as a cluster of inliers should not fit entirely into a single leaf node; there might  

%rank anomalies by 
%also exploit the distance $\mathtt{d}(\pointi, \point_{\mathtt{f}(\pointi)})$ between an object of interest $\pointi$ and its foreign representative $\point_{\mathtt{f}(\pointi)}$ 

%to the representative of 
%we propose to not only use the distance to the closest root object as the overall score, but also the distance to the closest leaf. 

%Then, we define that the distance from an object to its closest leaf, is the distance from it to the closest leaf representative ignoring the representative object of its own leaf. 
%As finding the closest amongst all leaves can be expensive, we use an approximation. 
%In this approximation we only consider the leaves that have the same parent node as the leaf the investigated object is in. 
%This means that we are only computing $\log_{c}$ s distances to find the closest leaf.
%Thus, with the overall score defined as below, we guarantee low outlierness for inliers which doesn't have a root object in their cluster. 
%This is because all inliers will, in almost every possible scenario, have another leaf close to them.

%As a consequence, one can expect that the most central object stored in the root node tends to be quite close to the most centralized object of the entire dataset, if not being exactly it.
%We could use the distance to the representative of the root node as a point of reference to find an overall outlier score, able to detect all types of outliers. 
%But, that would only be fine if there is only one cluster of inlier data. 
%If that is not the case and we have many inlier clusters, all of the inlier clusters that are far away from the central inlier cluster would have a high overall outlier score. 
%Because of this, as we want to make our scores adaptive to as many different scenarios of data distribution as possible, we propose the distance to the closest object in the root node as an overall score for all outliers. With that, we took the challenge of making the Slim-tree have at least one root object for every inlier cluster of the data. 
%In other words, when we measure the overall score, we will be measuring the distance from objects to their closest inlier cluster. 
%Like this, global and collective outliers distributed anywhere in the space are going to have larger scores than inliers. 
%The same can be concluded for local outliers around the inlier clusters, as they tend to be farther apart from the center of a inlier cluster than the inliers themselves.

%\begin{equation}
%OS=d_{root} \cdot d_{cleaf}
%\label{eq:overall_score}
%\end{equation}

%Include illustration

\vspace{-0.05in}
\subsubsection{Sequential Refinement of Rankings}
\label{ssec:refine}
%After turning C-AllOut robust to changes in cluster sizes by defining a singular value for Nl, making it parameterless, the next step is making it robust to the order of insertion of points inside the tree.
The tree structure that we leverage is built by a sequential insertion of the objects, and has its own heuristics to efficiently avoid unfortunate selections of node representatives that nonetheless may occur depending on the order in which the objects are given for insertion.
Next we describe
%This section describes 
how to improve the initial tree created by following a given order of objects, say, random insertion, into a fine-tuned tree created from a better ordering of the objects---making \method robust to any order of objects given for a dataset $\dataset$.

 %has its own heuristics to efficiently avoid unfortunate selections of node representatives; nevertheless, they rarely occur depending on the order in which the objects are given for insertion.
%The main challenge here is therefore to improve one initial tree created by following a given order of objects, say, random insertion, into a fine-tuned tree that is created from a better ordering of objects.

As can be seen in Lines~$1$-$9$ of Algo.~\ref{algorithm:main}, we propose to achieve this goal by performing a sequential refinement of rankings. 
Specifically, an initial tree $\tree$ is created by following a given order of objects $\rank$; then, $\tree$ is iteratively refined by exploiting the overall ranking $\orank$ produced from it. 
Note that function {\sc CreateTree($\dataset$, $\rank$)} in Line~$3$ of Algo.~\ref{algorithm:main} uses the \textit{reverse} order of $\rank$ to insert objects in $\tree$. 
The idea behind this procedure is to insert clear inliers first in $\tree$, so as to avoid the selection of an outlier to be a node representative.
As we showcase empirically in  Suppl. \S\ref{sec:sup_refinement}, only a handful of iterations is sufficient to refine the insertion order (and as a result the outlier ranking), as most outliers are typically detected even after the first round.


\hide{
Finally, it is worth noting that our experimental evaluation described in the upcoming Subsection~\reminder{\ref{bla}} indicates that a random insertion may be only marginally worse than our proposed order of insertion.
The sequential refinement of rankings does not modify the time complexity of \method, but still it increases runtime.
Thus, we consider the refinement to be an optional procedure, since ignoring it might be advantageous in some particular applications where marginally worse results are acceptable given a considerable gain in runtime. \rc{should we keep this last paragraph? It helps by saying that the tree is not much sensitive to the order of insertion; still, saying it diminishes our proposed sequential refinement.}
\la{yes this reads alarming re: runtime. although its runtime overhead is small. Maybe just say a few iterations is enough? - since in one round we are probably detecting most outliers.}
}

%Unfortunately, the Slim-tree is highly sensitive to the order of insertion of objects. The Slim-tree tries to avoid this by selecting the most centralized object as the representative of each node. This means that, when a split happens, the two new representatives are going to be the most centralized objects from both newly-created nodes. This two new representative are also the ones that are going to be promoted to the parent node. This means that, only representatives, or most centralized objects, are going to have the chance to become representatives of the parent node. This behavior is repeated across all levels of the Slim-tree. But, although objects can be promoted, they cannot be demoted. In summary, if an outlier object gets to the root of the tree by being the first one of its neighboring space to be inserted, it will be stuck in the root until the root is splitted in a manner that the outlier object do not get promoted. In this way, the object will go one level down not because it was demoted, but because the tree grew up one level above it. 

%It is a bad idea to expect ideal splits that can help to happen. Because of this, it is best to insert first objects that are as most inlier as possible. Outliers should be inserted last. We call a permutation of the dataset which leads to outliers being inserted last as a good permutation, or as the best permutation. The advantages of having a “ground-truth best permutation” and a “ground-truth worst permutation” were confirmed by using the available labels of some datasets to guide the insertion order. The Slim-tree built with objects labeled as outliers being inserted last was, in all scenarios, the best one. Although not having too much of a performance difference to a Slim-tree with a random permutation, the change was still significant enough to be worth investigating.

%Having decided that finding a best permutation before the tree was important, there are many ways of trying to handle that. A particularly good option, for not depending on methods other than our own, is to use our own overall score as a measure to sort the permutation. We have devised an iterative method in which multiple trees are built in sequence. Each tree takes as input the dataset sorted using the overall score of the previous tree. Algorithm \reminder{provide algorithm} shows the steps behind the iterative approach.

%\reminder{motivate/discuss how post-processing to do this task is non-trivial.}

\vspace{-0.05in}
\subsection{Outlier-type Focused Ranking of Objects}\label{sec:ranktypes}
Moving further from an overall ranking, we next describe
%This section describes 
how \method ranks outliers of each particular type; focusing 
%We first focus 
first on global outliers, and then the collective and local outlier ranking.

\vspace{-0.05in}
\subsubsection{Global Ranking of Outliers} \label{sec:global}

%This section presents our global ranking.
%It exploits 
Here we build on
the fact that the overall ranking 
by Eq. \eqref{eq:overall_score}
%described in Subsection~\ref{sec:overall} 
tends to rank global and collective outliers ahead of the other objects.
Recall that the overall ranking $\orank$ ranks each object according to its distance to the closest cluster of inliers.
Both global and collective outliers tend to be far away from any of such clusters;
distinctly, local outliers are close to at least one cluster, while the inliers themselves are even closer.
Consequently, we expect that  $\orank = ( r_1, r_2, \dots, r_n )$ sorts any two objects $\point{r_i}, \point{r_j} \in \dataset$ such that $i < j$ only when $\point{r_i}$ is either a global or a collective outlier, and $\point{r_j}$ is not.
Thus, the main challenge here is to differentiate the global outliers from the collective ones.

Fortunately, these two types of outliers can be distinguished: collective outliers have close neighbors; global ones do not.
%This line of thought leads us to present the global ranking $\grank$.
Building on Def.ns~\ref{definition:nn} and \ref{definition:nnd},  %and~\ref{definition:global}, 
we form the ranking $\grank$ of global outliers by combining
\begin{enumerate*}[label=(\alph*)]
\item 
the score $\oscorei$ of an object~$\pointi$, which is the core of our overall ranking; with
\item 
the normalized distance $\distnni$ between $\pointi$ and its nearest neighbor $\nni$, as shown in Eq. \eqref{eq:global}.
%distance $\distnni$ of $\pointi$ to its approximate nearest neighbor $\nni$.
\end{enumerate*}
Intuitively, score $\oscorename$ separates global and collective outliers from other objects, while distance $\distnnname$ differentiates outliers of these two types.
Note that the normalization
%\footnote{~Value $1$ in the denominator avoids divisions by near-zero; they disturb the results due to the limited precision of a machine.} 
 in %$\distnni$ 
 Eq. \eqref{eq:nnd}\footnote{Note that value $1$ in the denominator avoids division by zero.\label{note:division}}
 balances the distances according to the local neighborhood of~$\pointi$.
Also, the nearest neighbor $\nni$ is in fact an approximate one; it is efficiently obtained by comparing $\pointi$ only with the few objects in leaf $\leafi$. 
It tends to be a good approximation since our base tree is built to have each leaf storing only objects that are very similar to, i.e. nearby each other.
%using score $\oscore$ from the overall ranking combined with the distances of each object to  

\begin{Definition}[Approximate Nearest Neighbor]{
The approximate nearest neighbor $\nni$ of object $\pointi \in \dataset$ in a tree~$\tree$ is $\nni := \{\pointj \in \leafipoints \;|\; \arg\min_{j \neq i} \distij\}$, where $\leafipoints$ is the set of objects stored in leaf $\leafi$.
\label{definition:nn}
}\end{Definition}

\begin{Definition}[Normalized $1$nn Distance] {
%{\normalfont({\sc Normalized Distance to Nearest Neighbor})}
The normalized nearest neighbor distance $\distnni$ of an object $\pointi \in \dataset$ indexed in a tree~$\tree$ is defined as
\vspace{-0.05in}
\begin{equation}
\distnni = \frac{\dist{\pointi}{\nni}}{1 + \dist{\repi}{\nn{\leafi}}}
\label{eq:nnd}
\vspace{-0.1in}
\end{equation}
where $\nn{\leafi}~:=~\nnj$ s.t.  %\;|\; 
$\pointj$ is equivalent to $\repi$.
\label{definition:nnd}
}\end{Definition}

\begin{ranking}[\textbf{Global Ranking}]{
The global ranking $\grank = ( r_1, \dots, r_n )$ for dataset $\dataset$ is 
the ranking in which $\gscore{r_i} \geq \gscore{r_{i+1}} \ \forall i \in \{ 1,2,\dots, n-1\}$, where
%the global scoring function $\gscorename : \dX \xrightarrow{} \mathbb{R}$ is given by
\vspace{-0.05in}
\begin{equation}
 \gscorej = \oscorej \ \cdot \ \distnnj
 \label{eq:global}
\end{equation}
\label{definition:global}
\vspace{-0.3in}
}\end{ranking}




%As shown in section \ref{sec:back}, the Slim-tree is built using heuristics that create a tendency for the objects of the root node of the tree to be localized at the center, or most dense part, of the subsample of data that they represent. 
%Since the most dense area of the subsample distribution has the majority of the instances, it also has the most chances of having the root object. 
%Thus, we take that, root objects are a good point of reference to globally compare all objects indexed in its subtree (or subsample). 
%The global outliers are defined as the objects farthest from the center of the subsample of the dataset. 
%This outlierness is given to us by the Overall Score \textit{OS}. 
%Collective outliers can also be located far apart from the center of the subsample. 
%That being said, to achieve a score that puts global outliers separately above all other types, we additionally multiply \textit{OS} with the distance from the object to its nearest neighbor. 
%This should highlight only global outliers as collective outliers have small distances to their nearest neighboring object. 

%Equation \ref{eq:global_score} defines our global measure taking \textit{OS} from Equation \ref{eq:overall_score}:

%\begin{equation}
%GS=OS \cdot d_{1NN}
%\label{eq:global_score}
%\end{equation}

%Include illustration

\subsubsection{Collective Ranking of Outliers} \label{sec:collective}

%This section presents 
The ranking $\crank$ of  collective outliers
%It 
builds naturally from the ideas discussed in the previous section, %~\ref{sec:global},
where we exploit the tendency of global and collective outliers to have the highest scores $\oscorename$,
and then ``amplify'' each object $\pointi$ that is a global outlier by multiplying $\oscorei$ by the nearest neighbor distance $\distnni$.
In a similar fashion, we bump up collective outliers simply by replacing the multiplication with its reverse operation division\footref{note:division}, as
%Our proposed collective ranking of outliers $\crank$ is therefore 
presented in Eq. ~\eqref{eq:collective}.

\begin{ranking}[\textbf{Collective Ranking}]{
The collective ranking $\crank = (r_1,  \dots, r_n )$ for dataset $\dataset$ is the ranking in which $\cscore{r_i} \geq \cscore{r_{i+1}} \ \forall i \in \{ 1,\dots, n-1\}$, where
\vspace{-3mm}
\begin{equation}
 \cscorej = \frac{\oscorej}{1+\distnnj}
 \label{eq:collective}
\end{equation}
\label{definition:collective}
\vspace{-0.2in}
}\end{ranking}

%Collective outliers are groups of outlier instances that are near each other. Because of that, they tend to be indexed together in the same nodes by the Slim-tree. Collective outliers are also far away from inlier clusters, otherwise, since they are a group of objects, they would just be an appendix of an inlier cluster. Having that in mind, we can say that, for collective outliers, their distance to their closest inlier cluster, or overall score, is big. On the other hand, a collective outlier distance to its nearest neighboring object $d_{1NN}$ is small. For this reason, we can combine \textit{OS} with $d_{1NN}$ to get a collective score \textit{CS}. Therefore, Equation \ref{eq:collective_score} defines how we can take \textit{OS} and factor it by $d_{1NN}$ to make all local and global outliers have their score reduced, leaving only collective outliers with high outlierness.

%\begin{equation}
%CS=\frac{OS}{d_{1NN}}
%\label{eq:collective_score}
%\end{equation}

%Include illustration

%If the global score is divided by the local score, only the collective outliers are highlighted. This is because global outliers have big global and local scores, while local outliers have large  We call this metric collective score.

\subsubsection{Local Ranking of Outliers} \label{sec:local}

% The Split Methods behind the Slim-tree construction generates a tendency for the representative object of a node to be the centralized in relation to the objects it indexes. This happens when the objects are all distributed around the most centralized object when a split happens. In this manner, it is possible to use the representative as a point of reference to compare objects in a small subsample, locally. We select the objects with the longest distances to their representatives to be local outliers. As the clusters can have different densities, we normalize the distance to the representative object dividing it by the median distance to representative of all objects in the analyzed cluster. This metric is defined as the local score.

%Equation

%Include illustration

The local ranking of outliers $\lrank$ is formally given in Ranking~\ref{definition:local} below, which builds on Def.ns~\ref{definition:radius} and~\ref{definition:kneeradius}.


\begin{Definition}[Normalized Leaf Radius] {
The normalized leaf radius $\lradiusany$ of a leaf~$\leafname$ in a tree~$\tree$ is
\vspace{-2mm}
\begin{equation}
 \lradiusany = \frac{\dist{\repleaf}{\fnleaf}}{1 + \dist{\repleaf}{\nnleaf}}
\end{equation}
where $\fnleaf := \{\pointi \in \leafanypoints | \arg\max_i \dist{\repleaf}{\pointi}\}$
%$\fnleaf := \pointi~\in~\leafanypoints \ s.t. \ \arg\max_i \dist{\repleaf}{\pointi}$ 
is the farthest from the leaf representative
among objects $\leafanypoints$ in leaf $\leafname$, and 
$\nnleaf~:=~\nnj$ s.t. $\pointj$ is equiv. to $\repleaf$.
%$\nnleaf~:=~\{\nnj \;|\; \pointj = \repleaf \}$.
\label{definition:radius}
}\end{Definition}

\begin{Definition}[Knee Radius] {
The knee radius $\kneeradius$ for a dataset~$\dataset = \{\point{1}, \dots \point{n}\}$ in a tree~$\tree$ is defined as
\vspace{-1mm}
\begin{equation}
\kneeradius = \kneedle{\llradius{1}, \dots , \llradius{|\slradiuses|}}
\vspace{-1mm}
\end{equation}
s.t. $\slradiuses=\{\lradius{\leaf{1}}, \dots, \lradius{\leaf{n}}\}$,
%$\llradius{i} \in \slradiuses \ \forall i \in \{ 1,\dots, |\slradiuses|\}$, 
and
$\llradius{j} < \llradius{j+1} \ \forall j \in \{ 1,\dots, |\slradiuses|-1\}$. 
Function $\kneedlename$ refers to algorithm Kneedle~\cite{kneedle}; it takes a sorted list $\left(\llradius{1}, \dots , \llradius{|\slradiuses|}\right)$ as input and returns one of its values $\llradius{p}$.
\label{definition:kneeradius}
}\end{Definition}

\begin{ranking}[\textbf{Local Ranking}]{
The local ranking for dataset $\dataset$ is denoted by $\lrank$.
Let $\pointout = \{ \pointi \;|\; \distnni~\geq~\kneeradius \}$.
Then, $\lrank = (r_1,  \dots, r_n )$ is the ranking in which
\vspace{-1mm}
\begin{equation}
\point{r_j} \in 
\begin{cases}
    \pointout, \ \ \ \ \ \ \ \ \ \ if \ \ 1\leq j \leq |\pointout|\\
    \dataset\setminus\pointout, \ \ \ \ \ otherwise
    \vspace{-1mm}
\end{cases}
\end{equation}
where $\gscore{r_p} \leq \gscore{r_{p+1}} \ \forall p \in \{ 1,\dots, |\pointout|-1\}$ and
$\gscore{r_q}~\geq~\gscore{r_{q+1}} \ \forall q \in \{ |\pointout|+1,\dots, n-1\}$.
\label{definition:local}
}\end{ranking}

The main idea is to distinguish local outliers from other objects by using the normalized
%\footref{note:division} \la{is this pointing to the right thing??} \rc{yes, we use this footnote 3 times} 
leaf radius $\lradiusany$ of each leaf $\leafname \in \tree$.
%Note that the object $\fnleaf$ defining the radius~$\lradiusany$ is usually an outlier; unless there are only inliers in~$\leafname$.
Particularly, we expect $\lradiusany$ to be:
\begin{enumerate*}[label=(\alph*)]
\item small, if the object~$\fnleaf \in \dataset$ that defines the radius is an inlier;
\item larger, if $\fnleaf$ is a local outlier;
\item very large, if $\fnleaf$ is a global outlier;
 and
\item either very small or large\footnote{If the collective outliers are in a leaf of their own, $\lradiusany$ would be very small, and very large otherwise.}, if $\fnleaf$ is a collective outlier.
\end{enumerate*}
%\rc{an illustration would fit well here}

%This line of thought lead us to believe that 
As a result, the vast majority of leaf radii are expected to be small, mostly coming from case (a) and some from case (d) above, with only a few large radius leaves.
Thus, when the radii in $\slradiuses=\{\lradius{\leaf{1}}, \dots, \lradius{\leaf{n}}\}$ are sorted into a list $(\llradius{1}, \dots , \llradius{|\slradiuses|})$, there must exist a ``knee'' value/radius $\kneeradius$ that clearly separates the small radii from the rest.
Intuitively, $\kneeradius$ depicts the smallest distance $\distnni$ of each object $\pointi \in \dataset$ that is a local outlier.
Our Ranking~\ref{definition:local} 
computes $\kneeradius$ using an off-the-shelf ``knee''-detector algorithm; 
then, it separates large-radii outliers in set $\pointout$, and 
reuses our global score to rank them in increasing order of $\gscorename$, effectively placing local outliers ahead of the other objects. 
%\rc{an illustration would fit well here}

\subsection{Time and Space Complexity}

\begin{lemma}[Time Complexity]{The overall time complexity of \method is $O(n \log n )$.}\label{lemma:timecomplexity}
\end{lemma}
% \vspace{-0.2in}
% \begin{proof}
% See proof in Suppl. \S\ref{sec:sup_time_complexity}.
% \end{proof}
\vspace{-0.15in}
\begin{lemma}[Space Complexity]{The overall space complexity of \method is $O(n \log n )$.}\label{lemma:spacecomplexity}
\end{lemma}
\vspace{-0.1in}
\begin{proof}
See  Suppl. \S\ref{sec:sup_time_complexity} and \S\ref{sec:sup_space_complexity}, respectively.
\end{proof}

%\subsection{Optimizing Slim-tree’s structure for our needs \reminder{Making \method Parameter-free}}

%As the number of objects per leaf Nl changes, the way the Slim-tree covers the space becomes different. Having a smaller Nl means that more nodes, leaf and index, are needed to store all the objects. Larger Nl translates to a lesser amount of nodes needed. The choice of Nl impacts directly on C-AllOut final performance. If the leaf nodes are too small, the representatives are going to represent a not significant portion of data, the dataset will become overrepresented (Slim-tree overfits the data) and the scores will lose meaning. If the leaf nodes are too large, the representatives will cover too much data, including unrelated objects, the dataset will become underrepresented (Slim-tree underfits the data), there will be more overlapping between the nodes and the scores will also lose meaning. 

%The overlapping of nodes confuses the scores as single objects can be located in spaces covered by multiple nodes. Therefore, the leaf representative object may not be the ideal one. This would directly impact the local and collective scores, as both of them are relying on the distance, or median distance, to the representative object. Indirect impacts would also happen in the global score, as the root node would carry, and even boost, the overlapping of its child nodes.

%If we don’t want the tree to be overfitted or underfitted, we need to choose a reasonable medium-sized value for Nl. As the overlapping between becomes more dangerous on the initial levels of the tree and as the distance to the closest root is our most contributing score, we decided that developing a good heuristic for selecting a value for Nl should consider mainly the droot related scores. Any impacts on the other metrics should be considered secondary and evaluated as needed. In other words, the focus here is to choose a Nl that leads to a good number of root objects.

%Slim-tree’s structure is built in a way that every level of the tree, starting from object level, is reduced by a logarithmic factor until we reach the single root node of the tree. Because of this, we can estimate an upper bound for the number of nodes in every tree level, except for object level, using the equation:

%Nlupperbound = logNl(N / l)

%Where Nl is the maximum number of objects in every leaf; l is the current level of the tree, counting from object level and n is the number of objects currently stored in the tree.

%Note that this estimation, being an upper bound, considers that every node in the tree is full and ignores the fact that leaf nodes and index nodes don’t have the same size. In the same way, a lower bound for the number of nodes in every tree level can be estimated through the equation:

%Nllowerbound = logNl(N/1)
%    		= logNl(N)

%as the minimal amount of objects a node can have is 1, consisting of the representative object. There cannot be empty nodes.

%As we are aiming for a three-leveled tree (need to explain better the advantages of a three-leveled tree) the ideal Nl should be one that returns a value bounded in the following way:

%Equation

%The nodes of the tree are rarely full. There is nothing creating a tendency for them to be full or empty, except the natural insertion of new elements until the node splits. Then, we can say that node occupation is just dependent on a random probability. Because of this, if we were to take an educated guess on the occupation of a node, the best one is to pick a medium-sized occupation. When we suppose the node is at its half capacity we can reduce the amount of error that picking an extreme node occupation would give. For example, supposing all nodes are full would lead to large errors when they are empty and small errors would happen only if the node is full or a little bit empty. When a medium-sized occupation is picked, small errors can be achieved if we miss the occupation by a little bit below or over our estimate. Other than that, errors would never be as big as when we select extreme occupations (maybe illustration would help?). Finally, we estimate the best Nl value for our method using the following algorithm based on previous equations: (Algorithm needed).

==> paper_CatchOutAll copy/5_experiments.tex <==
\section{Evaluation} \label{sec:experiments}

We designed experiments to evaluate \method w.r.t. both overall detection as well as outlier annotation tasks, aiming to answer the following.
%This section presents the experiments and results for \method and its competitors. These are the two questions that guide the experiments.
\cbit
\item[\textbf{Q1:}] {\bf Overall detection performance:} How does \method compare to state-of-the-art (SOTA) baselines on benchmark datasets w.r.t. overall  detection performance, regardless of outlier type?
% Compared with four of the most recent and accurate outlier detectors in literature, how good is the overall ranking of \method?
\item[\textbf{Q2:}] {\bf Outlier annotation performance:} How well does \method perform on outlier annotation, that is,
w.r.t. its ranking of the outliers by type?
%How effective is the outlier tagging performance of \method against possible competitors methods?
\ceit

\vspace{-0.05in}
\subsection{Overall Detection Performance}

%This section investigates Question~\textbf{Q1}.


\subsubsection{Setup}
\vspace{-0.05in}
First we aim to showcase that, while specializing on outlier annotation, \method is competitive in terms of overall outlier detection on standard benchmark datasets compared to SOTA baselines.
We remark that \method's overall ranking $\orank$ is used for evaluation here, regardless of outlier type.

%Experiments were executed on a Intel(R) Xeon(R) CPU E7-4830 v3 @ 2.10GHz with 48 cores, 96 threads and 1 TB RAM. 


{\bf Testbed 1.~}
We create our first testbed using classical benchmark datasets\footnote{\url{http://odds.cs.stonybrook.edu/}}$^,$\footnote{\url{http://lapad-web.icmc.usp.br/repositories/outlier-evaluation/DAMI/}\label{note:repo2}}. 
Specifically, a total of $20$ datasets were chosen at random among those with outlier percentage less than 25\%; 
a detailed list of which is in Table \ref{tab:benchmark_datasets} in Suppl. \S\ref{sec:sup_dataset_summary}.


% Table \ref{tab:benchmark_datasets} in Supplementary Material \S\ref{sec:sup_dataset_summary} provides a summary on the selected datasets for Testbed 1, 2 and 3.


{\bf Baselines.~} We compare against four SOTA similarity or distance-based detection algorithms; namely, LOF \cite{lof}, kNN \cite{knn}, OCSVM \cite{scholkopf2000support}, and Sim-iForest (SIF, for short) \cite{czekalski2021similarity}. 
Specifically, LOF, kNN and SIF employ Euclidean distance and OCSVM uses the linear kernel.
Note that SIF is a version of the popular iForest \cite{liu2008isolation}, constructed by using pairwise similarities only based on ideas from similarity forests \cite{sathe2017similarity}.
(See Suppl. \S\ref{sec:sup_competitors_outlier_detection})


%competitors for \method in the task of outlier detection. One competitor that approaches the outlier annotation task marginally was also selected. Nonetheless, we have five competitors selected: LOF \cite{lof}, kNN \cite{knn}, OCSVM \cite{scholkopf2000support}, SIF \cite{czekalski2021similarity} for outlier detection; SRA \cite{nian2016auto} for outlier annotation, which is also similarity-based. 


%LOF, kNN and SIF use the Euclidean distance function, the same used for \method. OCSVM and SRA could not be trivially be adapted to work with the Euclidean distance. So, they work as originally proposed and use a similarity matrix, which is created from the dot product between the points.

Unlike \method, all baselines exhibit one or more hyperparameters (HPs) that are non-trivial to pick without any labels. We run each baseline using a corresponding list of HP configurations (See Table \ref{tab:sup_competitors_parameters} in Suppl. \S\ref{sec:sup_model_config}.) and report the average performance. In effect, this is equivalent to their expected performance when HPs are selected at random from the list. For the non-deterministic baseline SIF, the performance is averaged over 10 random runs.

%\la{revised until here. taking time...}All of our competitors can have different performances according to their hyperparameters. Using a list of hyperparameters that are feasible for each method, we report the average performance across different hyperparameter settings. This way, we are able to report the expected performance without uncertain hyperparameter tunning. \method's performance can also vary according to different configurations of the node capacity parameter. But, as there is a heuristic for estimating a good value for its hyperparameter, \method uses a single hyperparameter value for each dataset. \gs{it seems that we don't have the "making \method parameter-free" anymore, so this sentence can become too much superficial} A more detailed explanation of each competitor can be found in the supplementary material file. Reported AP and AUC values from non-deterministic methods are averages of 10 executions.

{\bf Measures.} We evaluate the outlier ranking quality using both AUC ROC curve and AUC Precision-Recall curve. %a.k.a. Average Precision (AP).
In addition, we apply the paired Wilcoxon signed rank test on AUC-ROC/PR results across datasets to establish statistical significance of the differences. 

%Two metrics are used in our experiments to make feasible to compare and test methods in different manners: Area Under the ROC Curve (AUC) and Average Precision (AP). Besides these metrics, we also apply the Wilcoxon signed-rank test on the AP and AUC results.

%\subsection{Testbed 1. Outlier Detection}
%\subsection{Overall Detection Performance}

%Tackling Q1, Testbed 1 aims to check how well does \method perform in detecting outliers in commonly used benchmark datasets for outlier detection. A summary of the used datasets can be found at the first section of Table \ref{tab:benchmark_datasets}.

%{\bf Detection Performance.~}

%We can check in Tables \ref{tab:auc_benchmark}, \ref{tab:ap_benchmark} that \textbf{\method is able to keep up and even outperform its competitors}. Having the average of AP and AUC from the tables in mind, together with the paired Wilcoxon signed-rank tests available in Table \ref{tab:wilcoxon}, we can see \textbf{\method being the second best performing method considering AUC and the best one considering AP}. Considering only AP values, \method comes very close to be significantly better than its best competitor, kNN. Note that \method's reported performance is related to its overall ranking.

%Additionally, we are able to assure that \textbf{\method also works as an outlier detection method that is parameter-free, not needing user input}. %Thus, \method is able to differentiate outliers from inliers and the overall ranking can indeed be used as base for other rankings.

\begin{table}[h]
\vspace{-0.05in}
    \scriptsize
    \caption{AUCROC performance on Testbed 1}
    \vspace{-0.1in}
    \begin{tabularx}{\columnwidth}{l|l|X|X|X|X} \hline
    Dataset & \method & LOF & kNN & OCSVM & SIF
    \\ \hline
    Annth. & 0.717 & 0.718 & \textbf{0.773} & 0.469 & 0.585
    \\
    Cardio & 0.528 & 0.535 & 0.503 & 0.380 & \textbf{0.795}
    \\
    Glass & \textbf{0.840} & 0.738 & 0.825 & 0.638 & 0.634
    \\
    Letter & 0.777 & \textbf{0.849} & 0.841 & 0.491 & 0.219
    \\
    Mammog. & 0.791 & 0.643 & \textbf{0.802} & 0.343 & 0.772
    \\
    Mnist & 0.848 & 0.662 & \textbf{0.852} & 0.408 & 0.585
    \\
    Musk & \textbf{0.954} & 0.555 & 0.795 & 0.415 & 0.919
    \\
    Optdigits & 0.465 & \textbf{0.506} & 0.437 & 0.504 & 0.372
    \\
    Pageb. & \textbf{0.903} & 0.712 & 0.877 & 0.523 & 0.852
    \\
    Pendigits & 0.848 & 0.517 & 0.813 & 0.615 & \textbf{0.879}
    \\
    Satim. & \textbf{0.998} & 0.639 & 0.961 & 0.527 & 0.894
    \\
    Shuttle & \textbf{0.986} & 0.851 & 0.953 & 0.374 & 0.765
    \\
    Shuttle2 & 0.786 & 0.517 & 0.701 & 0.647 & \textbf{0.963}
    \\
    Stamps & 0.807 & 0.643 & 0.856 & 0.530 & \textbf{0.859}
    \\
    Thyroid & 0.952 & 0.721 & \textbf{0.957} & 0.514 & 0.876
    \\
    Vowels & 0.932 & 0.885 & \textbf{0.953} & 0.549 & 0.317
    \\
    Waveform & 0.655 & 0.696 & \textbf{0.742} & 0.452 & 0.647
    \\
    WBC & 0.939 & 0.856 & \textbf{0.947} & 0.403 & 0.914
    \\
    WDBC & 0.904 & 0.831 & 0.923 & 0.474 & \textbf{0.927}
    \\
    Wilt & 0.463 & \textbf{0.635} & 0.541 & 0.296 & 0.299
    \\ \hline
    \textbf{Avg.} & 0.805 & 0.686 & \textbf{0.819} & 0.488 & 0.733
    \\ \hline
    \end{tabularx}
    \label{tab:auc_benchmark}
    \vspace{-0.25in}
\end{table}

\begin{table}[h]
    \scriptsize
    \caption{AUCPR performance on Testbed 1}
    \vspace{-0.1in}
    \begin{tabularx}{\columnwidth}{l|l|X|X|X|X} \hline
    Dataset & \method & LOF & kNN & OCSVM & SIF
    \\ \hline
    Annth. & \textbf{0.229} & 0.174 & 0.213 & 0.077 & 0.103
    \\
    Cardio & 0.322 & 0.272 & 0.312 & 0.209 & \textbf{0.582}
    \\
    Glass & 0.120 & \textbf{0.130} & 0.127 & 0.116 & 0.058
    \\
    Letter & 0.179 & \textbf{0.385} & 0.258 & 0.071 & 0.037
    \\
    Mammog. & 0.156 & 0.096 & 0.165 & 0.083 & \textbf{0.183}
    \\
    Mnist & 0.383 & 0.233 & \textbf{0.396} & 0.101 & 0.158
    \\
    Musk & \textbf{0.839} & 0.178 & 0.559 & 0.040 & 0.754
    \\
    Optdigits & 0.024 & 0.029 & 0.021 & \textbf{0.032} & 0.019
    \\
    Pageb. & \textbf{0.549} & 0.303 & 0.515 & 0.237 & 0.420
    \\
    Pendigits & \textbf{0.186} & 0.036 & 0.109 & 0.075 & 0.135
    \\
    Satim. & \textbf{0.938} & 0.050 & 0.583 & 0.108 & 0.170
    \\
    Shuttle & \textbf{0.323} & 0.220 & 0.271 & 0.011 & 0.027
    \\
    Shuttle2 & 0.290 & 0.101 & 0.182 & 0.317 & \textbf{0.776}
    \\
    Stamps & 0.255 & 0.186 & 0.283 & 0.258 & \textbf{0.289}
    \\
    Thyroid & \textbf{0.360} & 0.137 & 0.337 & 0.162 & 0.237
    \\
    Vowels & 0.347 & 0.320 & \textbf{0.477} & 0.076 & 0.021
    \\
    Waveform & 0.061 & 0.079 & \textbf{0.110} & 0.028 & 0.049
    \\
    WBC & 0.553 & 0.397 & 0.518 & 0.075 & \textbf{0.571}
    \\
    WDBC & 0.548 & 0.433 & 0.532 & 0.101 & \textbf{0.655}
    \\
    Wilt & 0.045 & \textbf{0.079} & 0.053 & 0.048 & 0.035
    \\ \hline
    \textbf{Avg.} & \textbf{0.335} & 0.192 & 0.301 & 0.111 & 0.264
    \\ \hline
    \end{tabularx}
    \label{tab:ap_benchmark}
    \vspace{-0.25in}
\end{table}


\subsubsection{Results}

Tables \ref{tab:auc_benchmark} and \ref{tab:ap_benchmark} respectively present the AUCROC and AUCPR overall detection performance results for all methods across all benchmark datasets.
In addition, Table  \ref{tab:wilcoxon} provides the $p$ values for one-sided significance tests of the differences, testing that the left-side method (\method) is better than the right-side (baseline) against the null that they are indifferent.
In terms of average AUCROC performance, \method significantly outperforms LOF, OCSVM and SIF and achieves on par with the top performer kNN (0.805 vs. 0.819) where the differences are not significant ($p\approx 0.5$).
Similar results hold for AUCPR, where \method achieves the largest average performance. The performance is comparable to kNN's (although $p$ value at 0.11 is relatively small) and significantly better than the rest.


\begin{table}[!t]
    \scriptsize
    \caption{Paired one-sided significance test (Wilcoxon): \method vs. baseline w.r.t. overall performance on Testbed 1. $p$-value in {\bf bold} if significant at 0.05.}
    \vspace{-0.1in}
    \begin{tabularx}{\columnwidth}{l|X|X} \hline
    Methods & AUCPR $p$-value & AUCROC $p$-value
    \\ \hline
    \method \textgreater \ LOF & \textbf{0.001163} & \textbf{0.001576}
    \\
    \method \textgreater \ kNN & 0.115256 & 0.492718
    \\
    \method \textgreater \ OCSVM & \textbf{0.000067} & \textbf{0.000002}
    \\
    \method \textgreater \ SIF & \textbf{0.048654} & \textbf{0.016384}
    \\ \hline
    \end{tabularx}
    \label{tab:wilcoxon}
    \vspace{-0.05in}
\end{table}

\subsection{Outlier Annotation Performance}
\vspace{-0.05in}

\subsubsection{Setup}
\vspace{-0.05in}
Next we aim to show the effectiveness of \method on annotating outliers by type, and specifically the accuracy of its type-specific rankings.
However, there exists no benchmark datasets with annotated outliers. %; that is, Testbed 1 datasets do not have a characterization of their outliers. 
To this end, we create two novel testbeds containing specific types of outliers, described as follows.



{\bf Testbed 2.~}
We start with simulating three synthetic base datasets, denoted S1, S2 and S3; consisting of Gaussian inlier clusters of varying count, size, standard deviation (std), and dimensionality. (See Table \ref{tab:synthetic_gen_parameters} in Suppl.) From each base dataset Sx, we create four versions: {Sx\_G}, {Sx\_L}, {Sx\_C}, and {Sx\_A} respectively with only global, only local, only collective, and all three types of outliers combined.
Global and local outliers are simulated from each inlier cluster by up-scaling the respective std, while each set of collective outliers are simulated from a point outlier as the mean and down-scaled std (See details in Suppl. \S\ref{sec:sup_gen_synthetic}.)



%{Sx\_A} all types of outliers; (2) \textbf{$\dataset$\_L}: variation having only local outliers; (3) \textbf{$\dataset$\_G}: variation having only global outliers; (4) \textbf{$\dataset$\_C}: variation having only collective outliers.

%In Testbed 2 we have three different base synthetic datasets, $S1, S2, S3$. Every variation carries the inliers from the base dataset $\dataset$ but has different configurations of outlier types: (1) \textbf{$\dataset$\_A}: variation having all types of outliers; (2) \textbf{$\dataset$\_L}: variation having only local outliers; (3) \textbf{$\dataset$\_G}: variation having only global outliers; (4) \textbf{$\dataset$\_C}: variation having only collective outliers.

%Every synthetic dataset is generated as multiple Gaussians clouds of points. The mean of each Gaussian is randomly put inside a predefined space. Every Gaussian has its own outliers that are generated using the Gaussian mean, but a different standard deviation. Table \ref{tab:base_datasets} in Supp. has a summary on synthetic datasets S1, S2 and S3.

{\bf Testbed 3.} We also create a testbed 
%with real-world data inliers, and simulated outliers 
based on Steinbuss and B{\"o}hm's ``realistic synthetic data'' generator
\cite{steinbuss2021benchmarking}.
The idea is to start with a real-world dataset containing only inliers, to which a Gaussian Mixture Model (GMM) is fit. Outliers are then simulated by up-scaling the variances of the GMM clusters. Their generator does not create collective outliers; to that end, we follow suit with Testbed 2 and simulate small-std micro-clusters centered at randomly chosen point outliers. (See details in Suppl. \ref{sec:sup_gen_realistic}.)
As the base, we use five real-world datasets (after discarding the (non-annotated) ground-truth outliers); namely  
%Testbed 3 has five base datasets, 
ALOI, Glass, skin, smtp, Waveform\footref{note:repo2} with various size and dimensionality % to represent different dataset characteristics 
(See Table \ref{tab:base_datasets} in Suppl. \S\ref{sec:sup_dataset_summary}). Similar to Testbed 2, we create 4 variants (\_G, \_L, \_C, \_A) from each base dataset with various types of (annotated) outliers.



%Each base dataset $\dataset$ gives birth to four variations. But, Testbed 3 goes beyond fully synthetic data. Using a realistic data generator capable of fitting Gaussian Mixtures to any inlier data. In this case, the inlier points of the base datasets are input into the generator so that it can learn their behavior. Original inliers are returned together with the newly simulated outliers at the end of the procedure. Only the simulated outliers are used and we discard original outliers as they cannot be trivially separated into local, global and collective outliers. 

%The five base datasets are selected to have a wide range of both number of points and features. This way, they can represent many different dataset characteristics. 

%As all original outliers were discarded, outlier ratio was not a choosing factor. Table \ref{tab:base_datasets} in Supp. presents a summary of the realistic base datasets, ALOI, Glass, skin, smtp and Waveform.





{\bf Baseline.} 
There is no baseline for annotating all three types of outliers. We found the spectral
SRA \cite{nian2016auto}, also based on pairwise similarities (i.e. Laplacian), as a close attempt (details in Suppl. \S\ref{sec:sup_competitors_outlier_annotation}). When it identifies a small cluster\footnote{SRA needs a size threshold for collective outliers; we give it an advantage by setting the threshold equal to the true size.}, it raises the flag ``clustered''  % the ranking to be for  (i.e. collective) outliers, and for 
and ``scattered'' otherwise. It provides a single ranking and does not distinguish between global and local outliers. Thus, SRA is only comparable in some cases.   




%{\bf Detection and Annotation Performance.~}


\begin{table*}[!th]
    \centering
    \scriptsize
    \caption{%\la{too much white space. can reduce col names and width. also thick black bars look ugly.}
    AUCROC performance on Testbed 2 with annotated outliers. Note that
    in Sx\_A datasets with all three outlier types, type-specific rankings are evaluated against outliers of the corresponding type only.
    %comparison between \method and SRA for outlier detection with overall ranking, as well as and annotation with separate rankings.}
    }
    \vspace{-0.1in}
    \begin{tabularx}{0.81\textwidth}{l|c @{\cspace} c|c @{\cspace} c|c @{\cspace} c|c @{\cspace} c} \hline
    Dataset & \method-$\orank$ & SRA & \method-$\lrank$ & SRA & \method-$\grank$ & SRA & \method-$\crank$ & SRA
    \\ \hline
    S1\_A & \textbf{0.997} & 0.663 & \textbf{0.999} & 0.452 & \textbf{1} & 0.851 & \textbf{0.999} & Not flagged
    \\
    S1\_L & \textbf{0.992} & 0.453 & \textbf{1} & 0.453 & - & - & - & -
    \\
    S1\_G & \textbf{1} & 0.851 & - & - & \textbf{1} & 0.851 & - & -
    \\
    S1\_C & \textbf{1} & 0.685 & - & - & - & - & \textbf{1} & Not flagged
    \\
    S2\_A & \textbf{1} & 0.703 & \textbf{0.997} & 0.511 & \textbf{1} & 0.747 & \textbf{1} & Not flagged
    \\
    S2\_L & \textbf{1} & 0.512 & \textbf{1} & 0.512 & - & - & - & -
    \\
    S2\_G & \textbf{1} & 0.744 & - & - & \textbf{1} & 0.744 & - & -
    \\
    S2\_C & \textbf{1} & 0.849 & - & - & - & - & \textbf{1} & Not flagged
    \\
    S3\_A & \textbf{1} & 0.599 & \textbf{0.998} & 0.567 & \textbf{1} & 0.729 & \textbf{1} & Not flagged
    \\
    S3\_L & \textbf{0.999} & 0.576 & \textbf{1} & 0.576 & - & - & - & -
    \\
    S3\_G & \textbf{1} & 0.730 & - & - & \textbf{1} & 0.730 & - & -
    \\
    S3\_C & \textbf{1} & 0.500 & - & - & - & - & \textbf{1} & Not flagged
    \\ \hline
    \end{tabularx}
    \label{tab:auc_synthetic}
    \vspace{-0.05in}
\end{table*}


%\subsection{Testbed 3. Outlier Annotation}


%{\bf Detection and Annotation Performance.~}




%Testbed 2 focuses on Q2 and provide information on how well \method do in a controlled environment. In Table \ref{tab:auc_synthetic}, we have provided a pairwise ranking comparison, between the overall, local, global and collective rankings of both \method and SRA. We can see that, in a fully-synthetic enviroment, \textbf{\method outperforms SRA in every dataset tested, in all the available rankings}. \method also does not make the mistake of not being able to correctly annotate types of outliers where only one type of outliers exist.



  
  %show the superiority of \method against its sole competitor SRA. \textbf{\method severely outperforms SRA in most of the scenarios evaluated, be it in outlier detection or annotation}. In SRA's columns of Table \ref{tab:auc_realistic}, ``Not tagged" cells show that the method was not able to note the existence of that type of outlier described in the name of the dataset. 

%Note that, differently from SRA, \method provides separate rankings. That being said, \textbf{no outlier type is missed because of the existence of another more numerous outlier type and \method never presents the ``Not tagged" status}. Nonetheless, we present the overall ranking for SRA that shows what would be the performance of the algorithm had we ignored its outlier type flag.

\begin{table*}[!t]
    \centering
    \scriptsize
    \caption{AUCROC performance on Testbed 3 with annotated outliers. Note that
    in variant \_A datasets with all three outlier types, type-specific rankings are evaluated against outliers of the corresponding type only.}
    \vspace{-0.1in}
    \begin{tabularx}{0.95\textwidth}{l|c @{\cspace} c|c @{\cspace} c|c @{\cspace} c|c @{\cspace} c} \hline
    Dataset & \method-$\orank$ & SRA & \method-$\lrank$ & SRA & \method-$\grank$ & SRA & \method-$\crank$ & SRA
    \\ \hline
    ALOI\_A & \textbf{1} & 0.474 & \textbf{0.993} & Not flagged & \textbf{1} & Not flagged & \textbf{0.996} & 0.429
    \\
    ALOI\_L & \textbf{1} & 0.908 & \textbf{1} & 0.908 & - & - & - & -
    \\
    ALOI\_G & \textbf{1} & 0.400 & - & - & \textbf{1} & Not flagged & - & -
    \\
    ALOI\_C & \textbf{1} & 0.429 & - & - & - & - & \textbf{1} & 0.429
    \\
    Glass\_A & \textbf{0.966} & 0.882 & \textbf{0.886} & 0.621 & \textbf{1} & 0.938 & \textbf{1} & Not flagged
    \\
    Glass\_L & \textbf{0.892} & 0.599 & \textbf{0.938} & 0.599 & - & - & - & -
    \\
    Glass\_G & \textbf{1} & 0.985 & - & - & \textbf{1} & 0.985 & - & -
    \\
    Glass\_C & \textbf{1} & 0.951 & - & - & - & - & \textbf{1} & Not flagged
    \\
    skin\_A & \textbf{0.999} & 0.868 & \textbf{0.994} & 0.730 & \textbf{1} & 0.864 & \textbf{0.999} & Not flagged
    \\
    skin\_L & \textbf{0.998} & 0.732 & \textbf{1} & 0.732 & - & - & - & -
    \\
    skin\_G & \textbf{1} & 0.869 & - & - & \textbf{1} & 0.869 & - & -
    \\
    skin\_C & \textbf{1} & 1 & - & - & - & - & \textbf{1} & Not flagged
    \\
    smtp\_A & \textbf{0.995} & 0.986 & \textbf{0.992} & 0.951 & \textbf{1} & 0.998 & \textbf{0.997} & Not flagged
    \\
    smtp\_L & \textbf{0.986} & 0.470 & \textbf{0.998} & 0.470 & - & - & - & -
    \\
    smtp\_G & \textbf{1} & 0.999 & - & - & \textbf{1} & 0.999 & - & -
    \\
    smtp\_C & \textbf{1} & 0.713 & - & - & - & - & \textbf{1} & Not flagged
    \\
    Waveform\_A & \textbf{1} & 0.575 & \textbf{0.991} & 0.512 & \textbf{1} & 0.480 & \textbf{1} & Not flagged
    \\
    Waveform\_L & \textbf{0.999} & 0.507 & \textbf{1} & 0.507 & - & - & - & -
    \\
    Waveform\_G & \textbf{1} & 0.491 & - & - & \textbf{1} & 0.491 & - & -
    \\
    Waveform\_C & \textbf{1} & 0.728 & - & - & - & - & \textbf{1} & Not flagged
    \\ \hline
    \end{tabularx}
    \label{tab:auc_realistic}
    \vspace{-0.1in}
\end{table*}

\vspace{-0.075in}
\subsubsection{Results}
Table \ref{tab:auc_synthetic} presents AUCROC results on Testbed 2. \method achieves near-ideal overall performance, while SRA ranking is significantly poor.
\method type-specific rankings continue to achieve near-perfect performance, while SRA struggles, especially in identifying local outliers with a near-random ranking. Moreover, it fails to flag ``clustered''  on datasets that contain collective outliers.
Results are similar w.r.t. AUCPR. (See Table \ref{tab:ap_synthetic} in Suppl.)



AUCROC results on the ``realistic synthetic'' Testbed 3 are shown in Table 
  \ref{tab:auc_realistic}.
\method achieves highly competitive performance and significantly outperforms SRA in all cases. Interestingly, type-specific rankings are better than the overall ranking for those specific outliers, which shows that they are effectively specialized. SRA fails to identify/flag the collective outliers, and in some other cases with scatter (local or global outliers) wrongly raises the ``clustered'' flag.
Results w.r.t. AUCPR are similar; see Table \ref{tab:ap_realistic} in Suppl.

==> paper_CatchOutAll copy/6_conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

We introduced \method, to our knowledge, the first approach that systematically tackles the outlier annotation problem. It provides not only an overall ranking but also a separate ranking by global, local, and collective
outlierness; all computed parameter-free and ``in-house'' (not post hoc), based on a scalable indexing tree structure.  
We showed
that \method is on par with or significantly outperforms state of the art outlier detectors on classical benchmark datasets. We also built two additional testbeds with annotated outliers and demonstrated the efficacy of \method in the annotation task.
To foster further work on this task, we open-source our testbeds and data generators along with the code for \method, at \url{https://bit.ly/3iUVwtM}.





\hide{
Outlier mining is a useful task for many applications, such as to identify network invasions, frauds in e-commerce, defective machinery in industry and even errors in data collection.
It has therefore a large literature.
Despite this popularity and the qualities of the existing works, we identified a key gap in the field: to our knowledge, no previous work addresses the \textit{outlier annotation problem}.
This paper tackled the problem by presenting \method: a novel algorithm that can not only effectively detect but also annotate the outliers as \textit{global}, \textit{local} or \textit{collective} ones.
We performed a comprehensive experimental evaluation, and showed that: when spotting outliers regardless of their type, \method\ achieves on par or significantly better performance compared with $4$ state-of-the-art detectors, namely, local-outlier factor, one-class SVM, nearest-neighbor based kNN, and ensemble based Isolation Forest. Additionally, we demonstrated that our proposed \method\ is highly effective at both detecting and annotating outliers of particular types, a task that none of the baselines can perform.

The annotations may provide valuable information to analysts for sense-making, triage and troubleshooting.
Global outliers are severe yet isolated cases that do not repeat; for example, a human mistake occurred when typing the value of an attribute.
Local outliers diverge from their peers within a context, like a particularly short basketball player that would not be seen as an outlier among the general population, or a cold day in the summer that could be seen as a regular day when together with days from other seasons.
Finally, collective outliers are isolated microclusters; they may indicate coalition or repetitions, thus being critical for settings like fraud detection. For example, in cybersecurity, collective outliers could be frauds that exploit the same loophole; or, reviews made by bots to illegitimately defame or promote a product in e-commerce.

Besides being able to annotate outliers by their type, \method\ exhibits several other desirable properties for practical use. 
It is parameter-free and scalable, also handling scenarios where only pairwise similarities (or distances) are available, instead of feature representations, still not being restricted to this setting. It is also capable of returning no outlier when there is none to be found, as opposed to many previous works. Finally, as we build on a dynamic data indexing structure that efficiently handles insertions and deletions of points without tree reconstruction, \method\ is 
naturally applicable to time-evolving or streaming settings where existing points may change or new points may arrive (or depart). With that in mind, as future work, we intend to investigate the use of \method\ in the streaming setting.
}

==> paper_CatchOutAll copy/dfn.tex <==


% \fgr{width = 0.50\textwidth}{FIG/duck.pdf}
\newcommand{\fgr}[3][\relax]{%
	\begin{figure}[htp]%
		\centering
		\includegraphics[#2]{#3}%
		\ifx\relax#1\else\caption{{#1}}\fi
	\end{figure}%
}

\usepackage{xcolor}
%\begin{figure}
%	\begin{tabular}{cc}
%		\centering
%		\includegraphics[width = 0.3\textwidth]{FIG/contour} &
%		\includegraphics[width = 0.50\textwidth]{FIG/TVsalesfit}  \\
%		(a) contours of least squares loss  & (b) least squares fit for regression of {\tt sales} onto {\tt TV}
%	\end{tabular}
%	\caption{xxx \label{fig:xxx}}
%\end{figure}

%\newcommand{\method}{{\sc CatchAllOut}\xspace}
\newcommand{\method}{{\sc C-AllOut}\xspace}

\newcommand{\etal}{{\it et al.}}


\definecolor{OliveGreen}{rgb}{0,0.6,0}
\newcommand{\tick}{\textcolor{OliveGreen}{\ding{52}}}



\newcommand{\BFSERIES}{\fontseries{b}\selectfont}



% datasets
\newcommand{\cora}{{\small{\tt Cora}}\xspace}
\newcommand{\cseer}{{\small{\tt Citeseer}}\xspace}
\newcommand{\pubmed}{{\small{\tt Pubmed}}\xspace}
\newcommand{\cauth}{{\small{\tt CoauthorCS}}\xspace}

\newcommand{\cbit}{\begin{compactitem}}
	\newcommand{\ceit}{\end{compactitem}}
\newcommand{\cben}{\begin{compactenum}}
	\newcommand{\ceen}{\end{compactenum}}

\newcommand{\bal}{\begin{align}}
\newcommand{\ean}{\end{align}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

%\newcommand{\mT}{\mathcal{T}}
%\newcommand{\mR}{\mathcal{R}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mL}{\mathcal{L}}

\newcommand{\mo}{\mathcal{o}}
\newcommand{\ml}{\mathcal{l}}

\newcommand{\hy}{\hat{y}}
\newcommand{\byy}{\mathbf{y}}
\newcommand{\bbx}{{\mathbf{\bar{x}}}}
\newcommand{\tbx}{{\mathbf{\tilde{x}}}}
\newcommand{\tbxo}{{\mathbf{\dot{x}}}}
\newcommand{\tbxi}{{\mathbf{\tilde{x}}}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bhy}{\mathbf{\widehat{y}}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bh}{\mathbf{h}}

\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bW}{\mathbf{W}}
%\newcommand{\bX}{\mathbf{X}}
%\newcommand{\bO}{\mathbf{O}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bN}{\mathbf{N}}
%\newcommand{\bR}{\mathbf{R}}


%\newcommand{\mO}{\mathcal{O}}
%\newcommand{\mN}{\mathcal{N}}

\newcommand{\dX}{\mathbb{X}}

\newcommand{\bH}{\mathbf{H}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\tbA}{\mathbf{\tilde{A}}}
\newcommand{\bAs}{{\mathbf{\tilde{A}}}_{\text{sym}}}
\newcommand{\bAl}{{\mathbf{\tilde{A}}}_{\text{rw}}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\tbD}{\mathbf{\tilde{D}}}
\newcommand{\bbX}{{\mathbf{\bar{X}}}}
\newcommand{\tbX}{{\mathbf{\tilde{X}}}}
\newcommand{\tbXi}{{\mathbf{\tilde{X}}}}
\newcommand{\tbXo}{\mathbf{\dot{{X}}}}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

%\newcommand{\mcF}{\mathcal{F}}
%\newcommand{\mcW}{\mathcal{W}}

\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bphi}{\boldsymbol{\Phi}}

\makeatletter
\algnewcommand{\LineComment}[1]{\Statex \hskip\ALG@thistlm \(\triangleright\) #1}
\makeatother


\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}
\newcommand{\la}[1]{{\textsf{\textcolor{purple}{[LA: #1]}}}}
\newcommand{\rc}[1]{{\textsf{\textcolor{orange}{[RC: #1]}}}}
\newcommand{\gs}[1]{{\textsf{\textcolor{green}{[GS: #1]}}}}
\newcommand{\todo}[1]{{\textsf{\textcolor{blue}{[TODO: #1]}}}}

\newcommand{\hide}[1]{}

\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{ranking}{Ranking}

\newcolumntype{?}{!{\vrule width 2pt}}

%%%%%%%%%%%%%%%% main notation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% data and distances
\newcommand{\dataset}{\mathbf{X}}
\newcommand{\point}[1]{\mathbf{x}_{#1}}
\newcommand{\pointref}[2]{\mathbf{x}^{#1}_{#2}}
\newcommand{\pointi}{\point{i}}
\newcommand{\pointj}{\point{j}}
\newcommand{\dist}[2]{\mathtt{d}(#1, #2)}
\newcommand{\distij}{\dist{\pointi}{\pointj}}

% tree
\newcommand{\tree}{\mathcal{T}}
\newcommand{\node}{\eta}
\newcommand{\rootnode}{\rho}
\newcommand{\rootpoints}{\mathbf{R}}
\newcommand{\leafname}{\tau}
\newcommand{\leaf}[1]{\leafname^{(#1)}}
\newcommand{\leafi}{\leaf{i}}
\newcommand{\leafj}{\leaf{j}}
\newcommand{\leafpointsname}{\mathbf{L}}
\newcommand{\leafpoints}[1]{\leafpointsname^{(#1)}}
\newcommand{\leafanypoints}{\leafpoints{\leafname}}
\newcommand{\leafipoints}{\leafpoints{i}}
\newcommand{\ant}[1]{\alpha_{#1}}
\newcommand{\antany}{\ant{\node}}
\newcommand{\anti}{\ant{\leafi}}
\newcommand{\antj}{\ant{\leafj}}
\newcommand{\rep}[1]{\pointref{(#1)}{\mathtt{e}}}
\newcommand{\repany}{\rep{\node}}
\newcommand{\repleaf}{\rep{\leafname}}
\newcommand{\repi}{\rep{\leafi}}
\newcommand{\croot}[1]{\pointref{(#1)}{\mathtt{r}}}
\newcommand{\crooti}{\croot{i}}
\newcommand{\crootj}{\croot{j}}
\newcommand{\frep}[1]{\pointref{(#1)}{\mathtt{f}}}
\newcommand{\frepi}{\frep{i}}
\newcommand{\frepj}{\frep{j}}
\newcommand{\nn}[1]{\pointref{(#1)}{\mathtt{nn}}}
\newcommand{\nnleaf}{\nn{\leafname}}
\newcommand{\nni}{\nn{i}}
\newcommand{\nnj}{\nn{j}}
\newcommand{\fn}[1]{\pointref{(#1)}{\mathtt{a}}}
\newcommand{\fnany}{\fn{\node}}
\newcommand{\fnleaf}{\fn{\leafname}}
\newcommand{\fni}{\fn{\leafi}}
\newcommand{\fnj}{\fn{\leafj}}
\newcommand{\distnnname}{\mathtt{d_{nn}}}
\newcommand{\distnn}[1]{\mathtt{d}^{(#1)}_{\mathtt{nn}}}
\newcommand{\distnni}{\distnn{i}}
\newcommand{\distnnj}{\distnn{j}}
\newcommand{\lradiusname}{\mathtt{a}}
\newcommand{\lradius}[1]{\lradiusname^{(#1)}}
\newcommand{\lradiusany}{\lradius{\leafname}}
\newcommand{\lradiusi}{\lradius{\leafi}}
\newcommand{\lradiusj}{\lradius{\leafj}}
\newcommand{\llradius}[1]{\lradiusname_{#1}}
\newcommand{\llradiusi}[1]{\lradiusname_{i}}
\newcommand{\llradiusj}[1]{\lradiusname_{j}}
\newcommand{\slradiuses}{\mathtt{A}}

% outliers and algorithm
\newcommand{\rank}{\mathcal{R}}
\newcommand{\orank}{\rank_o}
\newcommand{\grank}{\rank_g}
\newcommand{\lrank}{\rank_l}
\newcommand{\crank}{\rank_c}
\newcommand{\oscorename}{\mathtt{s_o}}
\newcommand{\oscore}[1]{\mathtt{s}^{(#1)}_{\mathtt{o}}}
\newcommand{\oscorei}{\oscore{i}}
\newcommand{\oscorej}{\oscore{j}}
\newcommand{\gscorename}{\mathtt{s_g}}
\newcommand{\gscore}[1]{\mathtt{s}^{(#1)}_{\mathtt{g}}}
\newcommand{\gscorei}{\gscore{i}}
\newcommand{\gscorej}{\gscore{j}}
\newcommand{\cscorename}{\mathtt{s_c}}
\newcommand{\cscore}[1]{\mathtt{s}^{(#1)}_{\mathtt{c}}}
\newcommand{\cscorei}{\cscore{i}}
\newcommand{\cscorej}{\cscore{j}}
\newcommand{\maxiter}{b}
\newcommand{\kneeradius}{\lradiusname_{\mathtt{kr}}}
\newcommand{\kneedlename}{\mathtt{kneedle}}
\newcommand{\kneedle}[1]{\kneedlename(#1)}
\newcommand{\pointout}{\mathbf{P}}

% table formatting
\newcommand{\cspace}{\hspace{1\tabcolsep}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> paper_CatchOutAll copy/symbols.tex <==
Table~\ref{tab:symbols} lists the main symbols used in our notation.

%---------------------------------------------------------------------
% Table of Symbols
%---------------------------------------------------------------------
\begin{table}[htb]
	\caption{Table of symbols.}  
	\label{tab:symbols}
	\centering
	\begin{tabular} {c|l} 
	  \hline
			\textbf{Symbols} & \textbf{Definitions} \\ \hline
			$X$ & A point-cloud dataset within domain $\mathbb{X}$. $X \subseteq \mathbb{X}$ \\
			$n$ & Number of instances in $X$, i.e. cardinality. $n=\left|X\right|$ \\
			$x_i$ & An instance from $X$. $x_i \in X$ \\
			$d$ & Distance function $d : \mathbb{X} \times \mathbb{X} \xrightarrow{} \mathbb {R}$. \\
			$d(x_i, x_j)$ & Distance between instances $x_i, x_j \in X$. \\
			$T$ & A Slim-tree created from $X$. \\
            $s$ & Size of $T$, i.e. total number of nodes. \\
            %$N$ & number of objects \\
            $h$ & Height of $T$, i.e. length of the longest path from the root. \\
            $l$ & Current tree level, i.e. the level of $T$ that is under \\ 
                & consideration at a given moment. $0 \leq l \leq h$ \\
            $c$ & Maximum node capacity for $T$. \reminder{leaf or index nodes?} \\
            %$Ni$ & maximum number of objects in index nodes \\
            $x_{cur}$ & Current instance, i.e. the one under consideration at \\
                      & a given moment. $x_{cur} \in X$\\
            $x_{rep}$ & Representative of the leaf node that stores $x_{cur}$ in $T$. \\
                      & $x_{rep} \in X$ \\
            $x_{crep}$ & Representative of the leaf node that is the closest to $x_{cur}$ in $T$. \\
                      & $x_{crep} \in X$ \\
            $x_{root}$ & Instance in the root node of $T$ that is the closest to $x_{cur}$. \\ 
                       & $x_{root} \in X$ \\
            $x_{1NN}$ & Instance in $T$ that is, approximately, the closest to $x_{cur}$. \\ 
                       & $x_{1NN} \in X$ \\
            $d_{rep}$ & Shortcut for $d(x_{cur}, x_{rep})$. \\
            $d_{root}$ & Shortcut for $d(x_{cur}, x_{root})$. \\
            $d_{crep}$ & Shortcut for $d(x_{cur}, x_{crep})$. \\
            $d_{1NN}$ & Shortcut for $d(x_{cur}, x_{1NN})$. \\
		\hline
	\end{tabular}
\end{table}
%---------------------------------------------------------------------

==> symbols.tex <==
Table~\ref{tab:symbols} lists the main symbols used in our notation.

%---------------------------------------------------------------------
% Table of Symbols
%---------------------------------------------------------------------
\begin{table}[htb]
	\caption{Table of symbols.}  
	\label{tab:symbols}
	\centering
	\begin{tabular} {c|l} 
	  \hline
			\textbf{Symbols} & \textbf{Definitions} \\ \hline
			$X$ & A point-cloud dataset within domain $\mathbb{X}$. $X \subseteq \mathbb{X}$ \\
			$n$ & Number of instances in $X$, i.e. cardinality. $n=\left|X\right|$ \\
			$x_i$ & An instance from $X$. $x_i \in X$ \\
			$d$ & Distance function $d : \mathbb{X} \times \mathbb{X} \xrightarrow{} \mathbb {R}$. \\
			$d(x_i, x_j)$ & Distance between instances $x_i, x_j \in X$. \\
			$T$ & A Slim-tree created from $X$. \\
            $s$ & Size of $T$, i.e. total number of nodes. \\
            %$N$ & number of objects \\
            $h$ & Height of $T$, i.e. length of the longest path from the root. \\
            $l$ & Current tree level, i.e. the level of $T$ that is under \\ 
                & consideration at a given moment. $0 \leq l \leq h$ \\
            $c$ & Maximum node capacity for $T$. \reminder{leaf or index nodes?} \\
            %$Ni$ & maximum number of objects in index nodes \\
            $x_{cur}$ & Current instance, i.e. the one under consideration at \\
                      & a given moment. $x_{cur} \in X$\\
            $x_{rep}$ & Representative of the leaf node that stores $x_{cur}$ in $T$. \\
                      & $x_{rep} \in X$ \\
            $x_{crep}$ & Representative of the leaf node that is the closest to $x_{cur}$ in $T$. \\
                      & $x_{crep} \in X$ \\
            $x_{root}$ & Instance in the root node of $T$ that is the closest to $x_{cur}$. \\ 
                       & $x_{root} \in X$ \\
            $x_{1NN}$ & Instance in $T$ that is, approximately, the closest to $x_{cur}$. \\ 
                       & $x_{1NN} \in X$ \\
            $d_{rep}$ & Shortcut for $d(x_{cur}, x_{rep})$. \\
            $d_{root}$ & Shortcut for $d(x_{cur}, x_{root})$. \\
            $d_{crep}$ & Shortcut for $d(x_{cur}, x_{crep})$. \\
            $d_{1NN}$ & Shortcut for $d(x_{cur}, x_{1NN})$. \\
		\hline
	\end{tabular}
\end{table}
%---------------------------------------------------------------------
